Bayesian Convolutional Deep Sets with Task-Dependent Stationary Prior

Convolutional deep sets are the architecture of a deep neural network (DNN) that can model stationary stochastic process. This architecture uses the kernel smoother and the DNN to construct the translation equivariant functional representations, and thus reflects the inductive bias of the stationarity into DNN. However, since this architecture employs the kernel smoother known as the non-parametric model, it may produce ambiguous representations when the number of data points is not given sufficiently. To remedy this issue, we introduce Bayesian convolutional deep sets that construct the random translation equivariant functional representations with stationary prior. Furthermore, we present how to impose the task-dependent prior for each dataset because a wrongly imposed prior forms an even worse representation than that of the kernel smoother. We validate the proposed architecture and its training on various experiments with time-series and image datasets.

==> 03-methodology-v04.tex <==







\section{Methodology}


% In this section, we first interpret the representation of the ConvDeepsets, and then present the motivation of our work in \cref{subsec:method1}. Then, we introduce how to build the task-dependent stationary prior in \cref{subsec:method2}, and the Bayesian ConvDeepsets in \cref{subsec:method3}. Last, we introduce how the Bayesian ConvDeepsets can be used for modeling the stationary process, and its training \cref{subsec:method4}.
% \textr{\cref{fig:main-illustration2} outlines how the Bayesian ConvDeepsets can be used to produce the predictive distributions on target sets. }


In this section, we first interpret the representation of the ConvDeepsets in \cref{subsec:method1}. Then, we introduce the task-dependent stationary prior in \cref{subsec:method2}, and the Bayesian ConvDeepsets in \cref{subsec:method3}. Last, we introduce the stationary process modeling via the Bayesian ConvDeepsets \cref{subsec:method4}.
\textr{\cref{fig:main-illustration2} outlines how the Bayesian ConvDeepsets models the predictive distributions on target sets. }






% \subsection{Interpretation of ConvDeepsets Representation} 
% \label{subsec:method1}
% %\paragraph{Interpretation of ConvDeepsets representation.}
% The data representation of $E(D^{c}) (\bigcdot)$ in \cref{eqn:convdeepset} is constructed by the kernel smoother, known as the non-parametric model. Thus, its expressive power is dependent on the $N^{c}$ context data points. In fact, when the lengthscale of the RBF Kernel function used in $E(D^{c})$ is chosen to be close to 0, the data channel of $E(D^{c}) (\bigcdot)$ represents the data only as follows:
% \begin{align}
% \sum_{n=1}^{N} \frac{y_n \ k(\bigcdot - x_n)}{ \sum_{n=1}^{N}  k(\bigcdot -  x_n) }
% \approx \sum_{n=1}^{N_c} y^{c}_n  \ \delta (\bigcdot -  x^{c}_n )
% \vspace{-2mm}
% \end{align}
% where $\delta(\bigcdot)$ is a Dirac-delta function. This implies that when $N^{c}$ context data points are not given sufficiently, the representation of data channel could be the ambiguous, and thus affect $\Phi(D^{c})(\bigcdot)$ negatively for modeling the predictive distribution $p(Y^{t} | X^{t},D^{c} )$.


% To remedy the issue, we reconsider the $E(D^{c})(\bigcdot)$, and note that its data channel can also be expressed as the re-scaled predictive mean of GP posterior with the restricted covariance $\text{Diag}(K(X^{c},X^{c}))$ as follows:
% \begin{align} 
% \frac{1}{\sum_{n=1}^{N^{c}}  k(\bigcdot -  x^{c}_n)} 
% \underbrace{ K(\bigcdot,X^{c}) \text{Diag}(K(X^{c},X^{c}))^{-1} Y^{c} }_{\mathrm{predictive \ mean \ of \ GP \ posterior}}  \label{eqn:interpretation} 
% \end{align}
% where $[\text{Diag}(K(X^{c},X^{c}))]_{n,m} =  1_{n=m}$ and $K(\bigcdot,X^{c}) \in R^{1 \times N^{c}}$. Based on this observation, we hypothesis that if we set the reasonable prior for each task $ \{ D^{c}, D^{t} \}$, and use or add the sample functions of the GP posterior for representing the data part in $E(D^{c})(\bigcdot)$, this could alleviate the unclear representation of the ConvDeepsets, that is caused from using small $N^{c}$ context data points. \cref{fig:concept} describes our concern of the data representation, and the following intuitive approach to remedy this issue.



% \begin{align}
% \sum_{n=1}^{N} \frac{y_n \ k(\bigcdot - x_n)}{ \sum_{n=1}^{N}  k(\bigcdot -  x_n) }
% \approx \sum_{n=1}^{N_c} y^{c}_n  \ \delta (\bigcdot -  x^{c}_n )
% \vspace{-2mm}
% \end{align}

\subsection{Interpretation of ConvDeepsets Representation} 
\label{subsec:method1}
%\paragraph{Interpretation of ConvDeepsets representation.}
The data representation of $E(D^{c}) (\bigcdot)$ in \cref{eqn:convdeepset} is constructed by the RBF kernel smoother known as the non-parametric model. \textr{The lengthscale of the RBF kernel controls the smoothness of data representation; when the lengthscale is close to 0, the data representation is expressed as $\sum_{n=1}^{N_c} y^{c}_n  \ \delta (\bigcdot -  x^{c}_n )$ with a Dirac-delta function $\delta(\bigcdot)$. This implies that the expressive power of kernel smoother is proportional to the number of context points $N^c$. When small $N^{c}$ context data is given, the data representation could be the ambiguous, and thus affect the $\Phi(D^{c})$ and the predictive distribution $p(Y^{t} | X^{t},D^{c} )$ negatively.}


To remedy the issue, we reconsider $E(D^{c})(\bigcdot)$ in \cref{eqn:convdeepset}, and note its data representation can also be expressed as the re-scaled predictive mean of GP posterior with the restricted covariance $\text{Diag}(K(X^{c},X^{c}))$, as follows:
\vspace{-2mm}
\begin{align} 
&\sum_{n=1}^{N} \frac{y_n \ k(\bigcdot - x_n)}{ \sum_{n=1}^{N}  k(\bigcdot -  x_n) } \label{eqn:interpretation}  \\
&= \frac{1}{\sum_{n=1}^{N^{c}}  k(\bigcdot -  x^{c}_n)} 
\underbrace{ K(\bigcdot,X^{c}) \text{Diag}(K(X^{c},X^{c}))^{-1} Y^{c} }_{\mathrm{predictive \ mean \ of \ GP \ posterior}}  \nonumber
\end{align}
where $[\text{Diag}(K(X^{c},X^{c}))]_{n,m} =  1_{n=m}$ and $K(\bigcdot,X^{c}) \in R^{1 \times N^{c}}$. Based on this observation, we hypothesis that if we set the reasonable stationary GP prior depending on each task, and use or add the sample functions of the GP posterior for representing the data part in $E(D^{c})(\bigcdot)$, this could alleviate the unclear representation of the ConvDeepsets, when using small $N^{c}$ context data points. \cref{fig:concept} describes our concern of the data representation for $E(D^c)$, and the following intuitive approach to remedy this issue.













%\begin{figure}[H]
\begin{figure}[t!]
\centering
%\subfloat[\label{fig:1d-singletask-a}  spectral density]
\subfloat[\label{fig:concept-1} Data representation of ConvDeepsets]
{\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/illustration_taskamiguity.pdf}} 

\vspace{1mm}
%\subfloat[\label{fig:1d-singletask-a}  spectral density]
\subfloat[\label{fig:concept-2} Data representation with stationary functional prior]
{\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/illustration_stationaryprior2.pdf}}   
\caption{Comparison of Data representation over different $N^{c}$ context points. \cref{fig:concept-1} shows the data representation of $E(D^{c})$ for ConvDeepsets; the black dots denotes the context set $D^{c}$, and black and blue line denote the true function and the data representation, respectively. \cref{fig:concept-2} shows the stationary priors characterized by each spectral density $p_{q}(s)$ in \cref{eqn:basiskernel}, and the improved data representation due to the reasonably imposed prior, especially for the $N^{c}=5$.
}
\label{fig:concept}
\end{figure}


\vspace{-2mm}
\subsection{Amortized Task-Dependent Stationary Prior}
\label{subsec:method2}



To impose the reasonable prior depending on the task, we employ an amortized latent variable approach for imposing the stationary prior. To this end, based on the Bochner's theorem \citeb{bochner1959lectures} that explains how the stationary kernel can be constructed through specifying the spectral density, we construct $Q$ stationary kernels $\{k_q\}_{q=1}^{Q}$ as follows:
\begin{align}
k_q(\tau) = \int e^{i 2\pi   s^{T} \tau}p_q(s) ds
\label{eqn:basiskernel}
\end{align}
where $p_q(s)$ denotes $q$-th spectral density defined on frequency domain. In this work, we model the spectral density  $p_q(s)=N(s;\mu_q,\mathrm{Diag}(\Sigma_q))$, and order the $\{k_q\}_{q=1}^{Q}$ by $\mu_1{=}0$ and $\mu_1 \leq .. \leq \mu_Q$ in element-wise sense. 




% \begin{figure*}[t!]
% \centering
% % {\includegraphics[width=0.99\linewidth]{Figures/03-methodology-explain01/bconvcnp_outline_v5.PNG}}   
% %{\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/tmp2.PNG}}   
% {\includegraphics[width=0.98\linewidth]{Figures/03-methodology-explain01/outline_v3.pdf}} 
% \caption{ Bayesian ConvDeepsets Forward Pass Outline: Step 0. the context set $D^{c}{=}\{(x^{c}_{n},y^{c}_{n})\}_{n=1}^{N_c}$ is given, Step 1. we first construct $N$ random functional representations by using \cref{eqn:samplez}, Step 2. we evaluate those $N$ functional representations on the finite grid $\mathcal{I} = \{t_{m} \}_{m=1}^{M}$, Step 3. we map those $N$ grid features by $p_{\mathrm{CNN}}$. Finally, we smooth the outputs of $p_{\mathrm{CNN}}$ on target set  $D^{t}{=}\{(x^{t}_{n},y^{t}_{n})\}_{n=1}^{N_t}$ as described in \cref{eqn:smoothed}, and then generate $N$ predictive distribution on target set as df.}
% \label{fig:main-illustration2}
% \end{figure*}


\begin{figure*}[t!]
\centering
% {\includegraphics[width=0.99\linewidth]{Figures/03-methodology-explain01/bconvcnp_outline_v5.PNG}}   
%{\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/tmp2.PNG}}   
{\includegraphics[width=0.98\linewidth]{Figures/03-methodology-explain01/outline_v3.pdf}} 
\caption{Prediction procedure of NP via using Bayesian ConvDeepsets: For the context set $D^{c}$ in step 1, the random data representations $\{RE(D^{c})\}_{n=1}^{N}$ in \cref{eqn:bayes_convdeepset} with the imposed prior are constructed in step 3; the prior (blue) is imposed out of the candidates of priors as shown in step 2, by $Z_{\mathrm{Cat}}$ of \cref{eqn:latentcat}. The (deterministic) data representation of ConvDeepsets can also be used together. Then, All representations are discretized, and mapped by CNN as shown in Step 4 and 5; here, the process of one representation is depicted for clarity. Then, they are used to make predictive distribution as shown in step 6.
}
\label{fig:main-illustration2}
\end{figure*}

\vspace{-2mm}

% In Step3, 

% Step 0. the context set $D^{c}{=}\{(x^{c}_{n},y^{c}_{n})\}_{n=1}^{N_c}$ is given, Step 1. we first construct $N$ random functional representations by using \cref{eqn:samplez}, Step 2. we evaluate those $N$ functional representations on the finite grid $\mathcal{I} = \{t_{m} \}_{m=1}^{M}$, Step 3. we map those $N$ grid features by $p_{\mathrm{CNN}}$. Finally, we smooth the outputs of $p_{\mathrm{CNN}}$ on target set  $D^{t}{=}\{(x^{t}_{n},y^{t}_{n})\}_{n=1}^{N_t}$ as described in \cref{eqn:smoothed}, and then generate $N$ predictive distribution on target set as df.


Then, we consider the categorical latent variable $Z_{\text{cat}} = (z_1,..,z_Q)$ parameterized by the neural network as follows:
\begin{align}
q(Z_{\text{cat}} \ | \ D^c) = \mathrm{Cat} \left( Z_{\text{cat}} \ ; \ \mathrm{p}_{\mathrm{nn}}(D^{c}) \right) \label{eqn:latentcat},
\end{align}
where $\mathrm{p}_{\mathrm{nn}}: D^c \longrightarrow {\Delta}^{Q-1} $, with $Q$-dimension simplex ${\Delta}^{Q-1}$, denotes the parameter of categorical variable parameterized by the translate invariant neural network satisfying 
\begin{align}
\vspace{-2mm}
\mathrm{p}_{\mathrm{nn}} (T_{\tau}(D^{c})) = \mathrm{p}_{\mathrm{nn}}(D^{c})  \label{eqn:transinv_net},
\end{align}
where $T_{\tau}(D^{c}) {=} \left((x^{c}_{1}+\tau,y^{c}_1), .., (x^{c}_{N^{c}}+\tau,y^{c}_{N^{c}}) \right) $ denotes the $\tau$-translated context set defined in \cref{def:TE}. This is considered to make the derived functional representation satisfy the TE as well, \textr{which will be stated in \cref{pro:Bayes_convdeepset}.} \textr{The structure of $\mathrm{p}_{\mathrm{nn}}$ in this work is described in Appendix}. 

Using the kernels $\{k_q(\tau) \}_{q=1}^{Q}$ in \cref{eqn:basiskernel} and the latent variable $Z_{\mathrm{cat}}(D^{c})$ in \cref{eqn:latentcat}, we build the amortized latent stationary kernel depending on the context set $D^{c}$ as
\begin{align}
k(\tau) \ | \ Z_{\text{cat}}(D^{c}) = z_1 k_1(\tau)  \hspace{2mm} +  \hspace{2mm} \cdots  \hspace{2mm}  + \hspace{2mm} z_Q k_Q(\tau).
\label{eqn:mixedkernel}
\end{align}
\paragraph{Multi-channel Extension.}  The latent stationary kernel in \cref{eqn:mixedkernel} can be extended for multi-channel processes ($K$ channels) by considering $K$ categorical variables $\{Z_{\text{cat}}^{k}(D^{c})\}_{k=1}^{K}$ with $Z_{\text{cat}}^{k}(D^{c}) \sim \mathrm{Cat}( \mathrm{p}^k (D^{c}) )$, where $\mathrm{p}^k (D^{c})$ denotes the amortized parameter for $k$-th channel.
\vspace{-2mm}
%\paragraph{Task-Dependent Stationary Prior}
\subsection{Bayesian Convolutional Deep sets.} 
\label{subsec:method3}
\vspace{-1mm}


Based on the latent stationary kernel in \cref{eqn:mixedkernel}, we build the random data representation, and the construct following Bayesian ConvDeepsets. To this end, we employ the path-wise sampling for GP posterior introduced in \citeb{wilson2020efficiently}. Let $f(D^c)(\bigcdot)$ be the random data representation for the context set $D^c = \{(x^{c}_n,y^{c}_{n})\}_{n=1}^{N^c}$, and it can be represented as 
% \begin{align}
% \underbrace{ f(D^c)(\bigcdot) }_{ \substack{\mathrm{random \ data} \\ \mathrm{representation}} } & \coloneqq \hspace{3mm} 
% \underbrace{\sum_{i=1}^{l} \textb{w_i}  \  \phi_i(\bigcdot)}_{\mathrm{prior \  term}}
% \hspace{2mm} + \hspace{1mm} 
% \underbrace{\sum_{n=1}^{N^{c}} \textb{v_{i}}  \ k(\bigcdot - x^{c}_{n} )}_{\mathrm{update \ term }},
% \label{eqn:randomfunctionalfeature}
% \end{align}
% where the prior term is computed as follows:
% \begin{align}
%  \{w_{i}\}_{i=1}^{l} &\sim N(0,I),   \label{eqn:mixed_fourier} \\
%  (z_{1},..,z_{Q}) & \sim q(Z_{\text{Cat}} \ | \ D^{c}),  \nonumber \\
%  \{s_{q,i}\}_{i=1}^{l} &\sim p_{q}(s), \hspace{2mm}
%  \{b_{q,i}\}_{i=1}^{l} \sim U[0,2\pi] , \hspace{2mm} q=1,..,Q   \nonumber  \\
%  \phi_i(\bigcdot) &= \sqrt{\frac{2}{l}} \sum_{q=1}^{Q} \sqrt{z_{q}} \  \cos{ ( 2 \pi \langle  s_{q,i}, \bigcdot \rangle + b_{q,i})} \nonumber.   
% \end{align}
\begin{align}
\hspace{-2mm}
\underbrace{ f(D^c)(\bigcdot) }_{ \substack{\mathrm{random \ data} \\ \mathrm{representation}} } & \coloneqq \hspace{3mm} 
\underbrace{\sum_{q=1}^{Q}\sqrt {z_q} \ \phi_q(\bigcdot) }_{\mathrm{prior \  term}} 
\hspace{.5mm} + \hspace{.5mm} 
\underbrace{\sum_{n=1}^{N^{c}} \textb{v_{i}}  \ k(\bigcdot - x^{c}_{n} )}_{\mathrm{update \ term }},
\label{eqn:randomfunctionalfeature}
\end{align}
where the prior term is computed as follows:
% \begin{align}
%  (z_{1},..,z_{Q}) & \sim q(Z_{\text{Cat}} \ | \ D^{c}), \label{eqn:mixed_fourier} \\
%   \{w_{i}\}_{i=1}^{l} &\sim N(0,I), \nonumber \\
%  \{s_{q,i}\}_{i=1}^{l} &\sim p_{q}(s), \hspace{2mm}
%  \{b_{q,i}\}_{i=1}^{l} \sim U[0,2\pi] , \hspace{2mm} q=1,..,Q   \nonumber  \\
%  \phi_q(\bigcdot) &= \sqrt{\frac{2}{l}} \sum_{i=1}^{l} w_{i} \cos{ ( 2 \pi \langle  s_{q,i}, \bigcdot \rangle + b_{q,i})} \nonumber.   
% \end{align}
\vspace{-1mm}
\begin{align}
 & (z_{1},..,z_{Q})  \sim q(Z_{\text{Cat}} \ | \ D^{c}), \hspace{3mm}
  \{w_{q,i}\}_{i=1}^{l} \sim N(0,I), \nonumber \\
 &\{s_{q,i}\}_{i=1}^{l} \sim p_{q}(s), \hspace{3mm}
 \{b_{q,i}\}_{i=1}^{l} \sim U[0,2\pi] , \hspace{1mm} q=1,..,Q   \nonumber  \\
 &\phi_q(\bigcdot) = \sqrt{\frac{2}{l}} \sum_{i=1}^{l} w_{q,i} \cos{ ( 2 \pi \langle  s_{q,i}, \bigcdot \rangle + b_{q,i})} \label{eqn:mixed_fourier}.   
\end{align}%\vspace{-1mm}
The \textb{\{$w_{i}\}_{i=1}^{l}$} denotes $l$ random weight samples. The $q(Z_{\text{Cat}} \ |\  D^{c})$ denotes the distribution of the amortized latent variable in \cref{eqn:latentcat}. The $\{p_{q}(s)\}_{q=1}^{Q}$ and $U[0,2\pi]$ denote the spectral density of the $k_q(\tau)$ in \cref{eqn:basiskernel} and the uniform distribution defined on $[0,2\pi]$, respectively. The $\{\phi_q(\bigcdot)\}_{q=1}^{Q}$ denotes the random stationary prior function of $\{k_q\}_{q=1}^{Q}$ kernels by using random Fourier feature (RFF) \citeb{rahimi2007random,jung2022efficient}. The update term for \cref{eqn:randomfunctionalfeature} is computed as follows:
\vspace{-.5mm}
\begin{align}
 k(\bigcdot - x^{c}_{i} ) &= \mathbb{E}_{ q(Z_{\text{cat}} \ | \ D^{c} ) }
 [  k(\bigcdot - x^{c}_{i} ) \ | \ Z_{\text{cat}}(D^{c})  ] \label{eqn:updateterm} \\ 
 v_{i} &= \left[  K(X^{c},X^{c}) {+} \sigma^{2}_{\epsilon}I  ) {}^{-1}
          \left(Y^{c} - \Psi(X^{c})W \right)  \right]_{i} \nonumber 
\end{align}
\vspace{-.5mm}
where the $k(\bigcdot - x^{c}_{i} )$ denotes the expected kernel of \cref{eqn:mixedkernel} over $q(Z_{\text{cat}}  | D^{C})$, and the \textb{$v_{i}$} denotes $i$-th element of the inversion term using the expected kernel Gram matrix $ K(X^{c},X^{c}) \in R^{N_c \times N_c} $ and \textr{the values of random stationary function on $X^{c}$}, i.e., $\Psi(X^{c})W \in R^{N_c} $ of which $i$-th element is evaluated by the prior term in \cref{eqn:randomfunctionalfeature} on $x^c_{i}$. 

\textr{Roughly speaking, the \cref{eqn:randomfunctionalfeature} can be understood as the generalization of the data representation of $E(D^{c})$ in sense that the random prior function using the expected kernel of \cref{eqn:mixedkernel} as the covariance is reflected on the representation.}


The \cref{eqn:randomfunctionalfeature} can be also approximated, i.e., $f(D^c)(\bigcdot) \approx$
\begin{align}
\hspace{-.5mm}
\alpha
\underbrace{  \sum_{q=1}^{Q} \textb{\sqrt{z_q}}   \phi_   q(\bigcdot)}_{\text{prior term}} +
\Tilde{k} * 
\Big(
\underbrace{
\sum_{n=1}^{N^{c}} y^{c}_n   \delta (\bigcdot -  x^{c}_n ) 
}_{\text{data term}}
- 
\alpha
\underbrace{
\sum_{q=1}^{Q} \textb{\sqrt{z_q}}   \phi_q(\bigcdot) 
}_{\text{prior term}}
\Big) \nonumber
\end{align}
for scalability, where the $\alpha \in (0,1)$ denotes the hyperparameter for controlling how much the stationary prior is reflected on $f(D^c)(\bigcdot)$. The $ \Tilde{k}$ denotes the truncated expected kernel in \cref{eqn:updateterm} with the finite length, and is used as the filter for smoothing the difference of data and prior values. This approximation works similarly as $f(D^c)(\bigcdot)$ in \cref{eqn:randomfunctionalfeature} reflects the stationary prior and the data term on the representation. In experiment, we validate that this alleviates the task ambiguity on the large-size image datasets empirically.


%\cref{eqn:randomfunctionalfeature}

% Additionally, we emphasize that the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D) (\bigcdot)$ has the following characteristic :
% \vspace{-1mm}
% \begin{itemize}[leftmargin=1em]
%     \vspace{-1mm}
%     \item \textbf{Flexibility:} The amortized latent stationary kernel \cref{eqn:mixedkernel} can assign the reasonable stationary prior if the target task can be modeled by the candidate of the stationary kernel $\{k_1,..,k_Q\}$. This is because $\{k_1,..,k_Q\}$ can construct any stationary kernel based on \cref{eqn:basiskernel}.
    
%     \vspace{-1mm}
%     \item \textbf{Generalization :} The random representation $f(D^{c})(\bigcdot)$ in \cref{eqn:randomfunctionalfeature} can be understood as the generalization of the data channel of $E(D^{c})$ in \cref{eqn:convdeepset}; note that if the random prior term is not considered and the RBF kernel is used for $f(D^{c})(\bigcdot)$, the $f(D^{c})(\bigcdot)$ represents the data channel of $E(D^{c})$. Thus, the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D) (\bigcdot)$ generalizes the ConvDeepsets the $\Phi (D) (\bigcdot)$.

    
%     \vspace{-0.5mm}
% \end{itemize}




Then, we can construct the random functional representation $RE(D) (\bigcdot)$ through the $f(D^{c})(\bigcdot)$ in \cref{eqn:randomfunctionalfeature}, and the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D^{c}) (\bigcdot) $ as the ConvDeepsets $\Phi (D^{c}) (\bigcdot) $ is constructed in \cref{pro:convdeepset} as follows:  
\vspace{-1mm}
\begin{align}
    \hspace{-0.5mm} 
       \underbrace{RE(D^{c}) (\bigcdot) }_{ \substack{ \mathrm{random \ functional} \\ \mathrm{representation} }    }  & =
    \Big[ \  
      \underbrace{\sum_{n=1}^{N^{c}}  k(\bigcdot -  x^{c}_n)}_{\mathrm{density}} 
          \hspace{3mm}  , \ 
         \underbrace{f(D^c)(\bigcdot) }_{ \substack{ \mathrm{random \ data} \\ \mathrm{representation}} }
          \
    \Big], \nonumber \\ 
 \underbrace{  \Phi^{\mathcal{B}} (D^{c}) (\bigcdot) }_{ \substack{ \mathrm{Bayes \ ConvDeepsets} \\ \mathrm{representation} }    }   & =
    \underbrace{ \rho}_{ \substack{ \mathrm{mapping \ via} \\ \mathrm{ CNN} } } 
    \circ 
    \underbrace{RE(D^{c}) (\bigcdot) }_{ \substack{ \mathrm{random  \ functional} \\ \mathrm{representation} }    }       
    \label{eqn:bayes_convdeepset} 
\end{align}


%  if the 
% e consider the translate invariant neural network satisfying 
% \begin{align}
% \mathrm{p}_{\mathrm{nn}} (T_{\tau}(D^{c})) = \mathrm{p}_{\mathrm{nn}}(D^{c}),
% \end{align}
In the following proposition, we prove that the Bayesian ConvDeepsets still holds the translation equivariance (TE):
\begin{proposition} 
\label{pro:Bayes_convdeepset}
Given the dataset $D=\{(x_n,y_n)\}_{n=1}^{N}$, if the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D) (\bigcdot)$ is defined on the finite grid points, $\Phi^{\mathcal{B}} (D) (\bigcdot)$ is still translation equivariant \textr{in distribution sense}, i.e.,
\begin{align}
\Phi^{\mathcal{B}}  \circ (T_{\tau}(D)) \stackrel{d}{=}  T^{*}_{\tau} \circ (\Phi^{\mathcal{B}}(D)).
\label{eqn:te_probsense}
\vspace{-3mm}
\end{align}

\begin{proof}
The detailed proof can be checked in \textr{Appendix A.3}.
\end{proof}
\vspace{-2mm}
\end{proposition}
% \textr{Roughly speaking,} the components of $f(D)(\bigcdot)$, defined by \cref{eqn:randomfunctionalfeature}, are consistently constructed in regardless of the translated dataset $T_{\tau}(D) = \{(x_n + \tau,y_n) \}_{n=1}^{N}$. The detailed proof can be checked in \textr{Appendix}.


\vspace{-2mm}





















\subsection{Prediction and Training}
\label{subsec:method4}


%\paragraph{Model.}
\paragraph{Prediction.} For the context set $D^{c}$ and target set $D^{t}$, 
the Bayesian ConvDeepsets can be used for computing predictive distribution $p(Y^{t}| X^{t}, D^{c} )$ as 
\begin{align}
& p(Y^{t}| X^{t}, D^{c} )  \label{eqn:prediction}\\
& =\int 
p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}  ) 
p(\Phi^{\mathcal{B}} | Z_{\text{Cat}},D^{c} )
\ p(Z_{\text{Cat}}| D^{c}  ) 
\ 
d \Phi^{\mathcal{B}}
d Z_{\text{Cat}}  \nonumber  \\
&\approx \frac{1}{N} \sum_{n=1}^{N} p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}_{(n)}  )  \nonumber
% {=} \frac{1}{N} \sum_{n=1}^{N} N(Y^{t}| \mu^{(n)}_{\text{nn}}(X^{t}), \sigma^{2(n)}_{\text{nn}}(X^{t})  ) \nonumber
\end{align}
where $Z_{\text{Cat}}$ denotes the categorical latent variable of \cref{eqn:latentcat} for choosing the stationary kernel. The $\Phi^{\mathcal{B}}$ denotes the representation of the Bayes ConvDeepsets $\Phi^{\mathcal{B}}(D^{c})(\bigcdot)$ evaluated on finite grid  $\mathcal{I} = \{t_m\}_{m=1}^{M}$ (see \cref{eqn:finite_convdeepset}), and $\Phi^{\mathcal{B}}_{(n)}$ denotes $n$-th random function sampled from $p( \Phi^{\mathcal{B}})$. The $p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}_{(n)}  )$ is modeled as 
\begin{align}
p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}_{(n)}  )= N(Y^{t}| \mu_{(n)}(X^{t}), \sigma^{2}_{(n)}(X^{t}) ), \nonumber
\end{align}
where the $n$-th predictive mean $\mu_{(n)}(X^{t})$ and standard deviation $\sigma^{2}_{(n)}(X^{t})$ on the target inputs $X^{t}$ are obtained by mapping the smoothed features of $X^{t}$ and $n$-th sample function $\Phi^{\mathcal{B}}_{(n)}$, as explained in \cref{eqn:smoothed}, via the neural network.







% \begin{figure*}[t]
% %\begin{figure}[htp!]
% \centering
% \subfloat[RBF]
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_rbf_v1.pdf}}   \hspace{0.1mm} 
% \subfloat[ Matern-${\frac{5}{2}}$] 
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_matern_v1.pdf}}   
% \subfloat[Weakly periodic]
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_weaklyperiodic_v1.pdf}}  \hspace{0.1mm} 
% \subfloat[Sawtooth]
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_sawtooth_v1.pdf}}   
% \caption{AAA}
% \label{fig:exp5-1:smallset_comparison}
% \end{figure*}






% \begin{figure*}[t]
% \subfloat[\label{fig:1d-singletask-a}  Spectral density]
% {\includegraphics[width=0.19\linewidth  ,height=2.40cm ]{Figures/05-experiments-task01/tmp0-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-b} RBF]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp1-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-c} Matern-${\frac{5}{2}}$]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp2-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-d} Weakly Periodic]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp3-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-e} Sawtooth]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp4-datav1.pdf}}  
% \vspace{1mm}
% \subfloat[\label{fig:1d-singletask-f} Prediction with \textr{$N^c=15$} context points]
% % {\includegraphics[width=0.99\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx8_bidx4_nc15_k4.pdf}}
% {\includegraphics[width=0.99\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx32_bidx0_nc15_k5.pdf}}
% \caption{Stochastic processes modeling beyond training range (gray region $[4,8]$): \cref{fig:1d-singletask-a,fig:1d-singletask-b,fig:1d-singletask-c,fig:1d-singletask-d,fig:1d-singletask-e} denote the trained spectral density of \cref{eqn:basiskernel} and $p_{\mathrm{nn}}(D^{c})$ of \cref{eqn:transinv_net} for each process, and \cref{fig:1d-singletask-f} denotes the prediction for the task of each process.}
% \label{fig:1d-singletask-prediction}
% \end{figure*}
% \vspace{-1mm}



\begin{figure*}[t]
\subfloat[\label{fig:1d-singletask-a}  Spectral density]
{\includegraphics[width=0.19\linewidth  ,height=2.6cm ]{Figures/05-experiments-task01/density_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-b} RBF]
{\includegraphics[width=0.19\linewidth ,height=2.6cm ]{Figures/05-experiments-task01/rbf_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-c} Matern-${\frac{5}{2}}$]
{\includegraphics[width=0.19\linewidth ,height=2.6cm ]{Figures/05-experiments-task01/matern_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-d} Weakly Periodic]
{\includegraphics[width=0.19\linewidth ,height=2.6cm ]{Figures/05-experiments-task01/weaklyperiodic_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-e} Sawtooth]
{\includegraphics[width=0.19\linewidth ,height=2.6cm ]{Figures/05-experiments-task01/sawtooth_datav1.pdf}}  
\vspace{1mm}
\subfloat[\label{fig:1d-singletask-f} Prediction with \textr{$N^c=15$} context points]
% {\includegraphics[width=0.99\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx8_bidx4_nc15_k4.pdf}}
{\includegraphics[width=0.99\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx32_bidx0_nc15_k5.pdf}}
\caption{Stochastic processes modeling beyond training range (gray region $[4,8]$): \cref{fig:1d-singletask-a,fig:1d-singletask-b,fig:1d-singletask-c,fig:1d-singletask-d,fig:1d-singletask-e} denote the trained spectral density of \cref{eqn:basiskernel} and $p_{\mathrm{nn}}(D^{c})$ of \cref{eqn:transinv_net} for each process, and \cref{fig:1d-singletask-f} denotes the prediction for the task of each process.}
\label{fig:1d-singletask-prediction}
\end{figure*}
\vspace{-1mm}


















% Let $\Theta$ be the learnable parameters for kernels $\{k_q\}_{q=1}^{Q}$ of \cref{eqn:basiskernel}, the noise parameters $\sigma_{\epsilon}$, $p_{\mathrm{nn}}$ of \cref{eqn:transinv_net}, and the CNN $\rho$ of \cref{eqn:bayes_convdeepset}. 



\paragraph{Training.} Let $\Theta$ be the learnable parameters for kernels, the translate invariant network, and the CNN. Then, using the meta-learning and variational inference \citeb{burda2016importance}, we maximize the following objective 
with respect to $\Theta$ as follows:
\begin{align}
 \mathbb{E}_{D^{c},D^{t} \sim p(\mathcal{T})} 
 \bigl[
 \mathcal{L}_{\text{ll}}(\Theta ; D^{c}, D^{t})  - \beta \hspace{.2mm} \mathcal{L}_{\text{reg}}( \Theta ;D^{c}, D^{t}) 
 \bigr]
\label{eqn:tr_objective}
\end{align}
where $\mathcal{L}_{\text{ll}}(\Theta ; D^{c}, D^{t})$ denotes the multi-sampled estimator of likelihood and $\mathcal{L}_{\text{reg}}(\Theta;D^{c}, D^{t})$ denotes the regularizer for the amortized latent variable $Z_{\text{cat}}(D^{c})$.

The likelihood $\mathcal{L}_{\text{ll}}(\Theta ; D^{c}, D^{t})$ is expressed as 
% \begin{align}
% &\mathcal{L}_{\text{ll}}(\Theta ; D^{c}, D^{t})  = \nonumber \\
% &
% \log{
% \left(
%  \frac{1}{N} 
%  \sum_{n=1}^{N} \exp{ \left(  \sum_{i=1}^{N^{t}} \log{p \left(  y^{t}_{i}| x^{t}_{i}, \Phi^{\mathcal{B}}_{(n)}  \right)}  \right) }   
%  \right)  
%  }   \nonumber
% \end{align}
\begin{align}
\log{
\left(
 \frac{1}{N} 
 \sum_{n=1}^{N} \exp{ \left(  \sum_{i=1}^{N^{t}} \log{p \left(  y^{t}_{i}| x^{t}_{i}, \Phi^{\mathcal{B}}_{(n)}  \right)}  \right) }   
 \right)  
 }   \nonumber
\end{align}

In this procedure, we use the Gumbel-softmax trick \citeb{jang2016categorical}, for $Z_{\text{Cat}}$ in \cref{eqn:latentcat} and reparametrization trick \citeb{jung2022efficient} for the prior term in \cref{eqn:randomfunctionalfeature}. These tricks enables end-to-end training, based on the automatic differentiation.


The regularizer $\mathcal{L}_{\text{reg}}(\Theta;D^{c}, D^{t})$ is expressed as 
% \begin{align}
% \mathcal{L}_{\text{reg}}(\Theta;D^{c}, D^{t})= \mathrm{KL} \left( q(Z_{\text{cat}} \ | \  D^{c} )  \ || \  p (Z_{\text{cat}} \ | \  D^{c}, D^{t}  )  \right) \nonumber
% %\label{eqn:reg-kl-zat}
% \end{align}
\begin{align}
\mathrm{KL} \left( q(Z_{\text{cat}} \ | \  D^{c} )  \ || \  p (Z_{\text{cat}} \ | \  D^{c}, D^{t}  )  \right) \nonumber
%\label{eqn:reg-kl-zat}
\end{align}
where $q(Z_{\text{cat}} \ | \  D^{c} )$  denotes the amortized categorical variable defined in \cref{eqn:latentcat}. The $ p (Z_{\text{cat}} \ | \  D^{c}, D^{t} ) $ denotes the posterior distribution of $Z_{\text{cat}}$, which will be used as the prior distribution for training $q(Z_{\text{cat}} \ | \  D^{c} )$; note $p (Z_{\text{cat}} \ | \  D^{c}, D^{t} )$ can be computed only during training phase.

%e k-dimensional sample vectors y ∈ ∆k−1

The posterior $ p (Z_{\text{cat}} \ | \  D^{c}, D^{t}  )= \mathrm{Cat}(Z_{\text{cat}};\mathrm{p}_{\mathrm{prior}}  ) $ is computed with the parameter $\mathrm{p}_{\mathrm{prior}} \in {\Delta}^{Q-1} $ of which $q$-th element $(\mathrm{p}_{\mathrm{prior}})_{q} $ is defined as follows: 
\begin{align}
(\mathrm{p}_{\mathrm{prior}})_{q} = 
\frac{\mathrm{exp} \left( \log{p(Y^{t} | X^{t}, D^{c}, k_q)} \ / \  \tau_{0} \right)}
{\sum_{q=1}^{Q} \mathrm{exp} \left( \log{p(Y^{t} | X^{t}, D^{c}, k_q)} \ /\  \tau_{0} \right)}
\end{align}
where $\tau_{0}$ denotes the tempering parameters. The $q$-th marginal likelihood $p(Y^{t} | X^{t},D^{c}, k_q)$, using the $q$-th stationary kernel $k_q$, is computed as
\begin{align}
\hspace{-2.2mm}
p(Y^{t} | X^{t},D^{c}, k_q) = N( Y^{t} ;\hat{\mu}_{q}(X^{t}),\mathrm{Diag}(\hat{\Sigma}_{q}(X^{t})) ) 
\label{eqn:emp-gpposterior}
\end{align}
where $\hat{\mu}_{q}(X^{t}) \in R^{N_t}$ and $\mathrm{Diag}(\hat{\Sigma}_{q}(X^{t})) \in R^{N_t}$ denote the empirical predictive mean and diagonal covariance of the GP posterior distribution on target set $X^{t}$. The sample functions of GP posterior, described in \cref{eqn:randomfunctionalfeature}, are used. The derivation of training loss is explained in \textr{Appendix A.1}.






==> 03-methodology-v05.tex <==




% %--------------------------------------------------------------------------
% %page 3 outline fig
% %--------------------------------------------------------------------------
% \begin{figure*}[t!]
% \centering
% {\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/outline_v3.pdf}} 
% \caption{Prediction procedure of NP via using Bayesian ConvDeepsets: For the context set $D^{c}$ in step 1, the random data representations $\{RE(D^{c})\}_{n=1}^{N}$ in \cref{eqn:bayes_convdeepset} with the imposed prior are constructed in step 3; the prior (blue) is imposed out of the candidates of priors as shown in step 2, by $Z_{\mathrm{Cat}}$ of \cref{eqn:latentcat}. The (deterministic) data representation of ConvDeepsets can also be used together. Then, All representations are discretized, and mapped by CNN as shown in Step 4 and 5; here, the process of one representation is depicted for clarity. Then, they are used to make predictive distribution as shown in step 6.
% }
% \label{fig:main-illustration2}
% \end{figure*}




\section{Methodology}


% In this section, we first interpret the representation of the ConvDeepsets, and then present the motivation of our work in \cref{subsec:method1}. Then, we introduce how to build the task-dependent stationary prior in \cref{subsec:method2}, and the Bayesian ConvDeepsets in \cref{subsec:method3}. Last, we introduce how the Bayesian ConvDeepsets can be used for modeling the stationary process, and its training \cref{subsec:method4}.
% \textr{\cref{fig:main-illustration2} outlines how the Bayesian ConvDeepsets can be used to produce the predictive distributions on target sets. }


In this section, we first interpret the representation of the ConvDeepsets and the following motivation in \cref{subsec:method1}. Then, we introduce the task-dependent stationary prior in \cref{subsec:method2}, and the Bayesian ConvDeepsets in \cref{subsec:method3}, and its application to stationary process modeling in \cref{subsec:method4}.
\textr{\cref{fig:main-illustration2} outlines the prediction procedure via Bayesian ConvDeepsets described in \cref{subsec:method2,subsec:method3,subsec:method4}.}




\subsection{Interpretation of ConvDeepsets Representation} 
\label{subsec:method1}
%\paragraph{Interpretation of ConvDeepsets representation.}
The data representation of $E(D^{c}) (\bigcdot)$ in \cref{eqn:convdeepset} is constructed by the RBF kernel smoother known as the non-parametric model. The lengthscale of the RBF kernel controls the smoothness of data representation; when the lengthscale is close to 0, the data representation is expressed as $\sum_{n=1}^{N_c} y^{c}_n  \ \delta (\bigcdot -  x^{c}_n )$ with a Dirac-delta function $\delta(\bigcdot)$. This implies that the expressive power of kernel smoother is proportional to the number of context points $N^c$. When small $N^{c}$ context data is given, the data representation could be the ambiguous, and thus affect the $\Phi(D^{c})$ and the predictive distribution $p(Y^{t} | X^{t},D^{c} )$ negatively.


% To remedy the issue, we reconsider $E(D^{c})(\bigcdot)$ in \cref{eqn:convdeepset}, and note its data representation can also be expressed as the re-scaled predictive mean of GP posterior with the restricted covariance
% $\text{Diag}(K(X^{c},X^{c}))$, as follows:

% To remedy the issue, we note its data representation of $E(D^{c})(\bigcdot)$ in \cref{eqn:convdeepset} can also be expressed as the re-scaled predictive mean of GP posterior with the restricted covariance
% $\text{Diag}(K(X^{c},X^{c}))$, as follows:
To remedy the issue, we note the data representation of $E(D^{c})(\bigcdot)$ in \cref{eqn:convdeepset} can also be expressed as the re-scaled predictive mean of GP posterior with the restricted covariance
$\text{Diag}(K(X^{c},X^{c}))$, as follows:
\vspace{-2mm}
\begin{align} 
&\sum_{n=1}^{N} \frac{y_n \ k(\bigcdot - x_n)}{ \sum_{n=1}^{N}  k(\bigcdot -  x_n) } \label{eqn:interpretation}  \\
&= \frac{1}{\sum_{n=1}^{N^{c}}  k(\bigcdot -  x^{c}_n)} 
\underbrace{ K(\bigcdot,X^{c}) \text{Diag}(K(X^{c},X^{c}))^{-1} Y^{c} }_{\mathrm{predictive \ mean \ of \ GP \ posterior}}  \nonumber
\end{align}
where $[\text{Diag}(K(X^{c},X^{c}))]_{n,m} =  1_{n=m}$ and $K(\bigcdot,X^{c}) \in R^{1 \times N^{c}}$. Based on this observation, we hypothesis that (1) setting the reasonable stationary GP prior depending on each task, and (2) using or adding the sample functions of the GP posterior for representing the data part in $E(D^{c})(\bigcdot)$ could alleviate the unclear representation of the ConvDeepsets, when using small $N^{c}$ context data points. \cref{fig:concept} describes our concern of the data representation for $E(D^c)$, and the following intuitive approach to remedy this issue.



% we hypothesis that if we set the reasonable stationary GP prior depending on each task, and use or add the sample functions of the GP posterior for representing the data part in $E(D^{c})(\bigcdot)$, this could alleviate the unclear representation of the ConvDeepsets, when using small $N^{c}$ context data points. \cref{fig:concept} describes our concern of the data representation for $E(D^c)$, and the following intuitive approach to remedy this issue.













%\begin{figure}[H]
\begin{figure}[t!]
\centering
%\subfloat[\label{fig:1d-singletask-a}  spectral density]
\subfloat[\label{fig:concept-1} Data representation of ConvDeepsets]
{\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/illustration_taskamiguity.pdf}} 

\vspace{1mm}
%\subfloat[\label{fig:1d-singletask-a}  spectral density]
\subfloat[\label{fig:concept-2} Data representation with stationary functional prior]
{\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/illustration_stationaryprior2.pdf}}   
\caption{Comparison of Data representation over different $N^{c}$ context points. \cref{fig:concept-1} shows the data representation of $E(D^{c})$ for ConvDeepsets; the black dots denotes the context set $D^{c}$, and black and blue line denote the true function and the data representation, respectively. \cref{fig:concept-2} shows the stationary priors characterized by each spectral density $p_{q}(s)$ in \cref{eqn:basiskernel}, and the improved data representation due to the reasonably imposed prior, especially for the $N^{c}=5$.
}
\label{fig:concept}
\end{figure}


\vspace{-2mm}
\subsection{Amortized Task-Dependent Stationary Prior}
\label{subsec:method2}



To impose the reasonable prior depending on the task, we employ an amortized latent variable approach for imposing the stationary prior. To this end, based on the Bochner's theorem \citeb{bochner1959lectures} that explains how the stationary kernel can be constructed through specifying the spectral density, we construct $Q$ stationary kernels $\{k_q\}_{q=1}^{Q}$ as follows:
\begin{align}
k_q(\tau) = \int e^{i 2\pi   s^{T} \tau}p_q(s) ds
\label{eqn:basiskernel}
\end{align}
where $p_q(s)$ denotes $q$-th spectral density defined on frequency domain. In this work, we model the spectral density  $p_q(s)=N(s;\mu_q,\mathrm{Diag}(\Sigma_q))$, and order the $\{k_q\}_{q=1}^{Q}$ by $\mu_1{=}0$ and $\mu_1 \leq .. \leq \mu_Q$ in element-wise sense. 



% the random data representations $\{RE(D^{c})\}_{n=1}^{N}$ in \cref{eqn:bayes_convdeepset} with the imposed prior are constructed in step 3; the prior (blue) is imposed out of the candidates of priors as shown in step 2, by $Z_{\mathrm{Cat}}$ of \cref{eqn:latentcat}. The (deterministic) data representation of ConvDeepsets can also be used together. Then, All representations are discretized, and mapped by CNN as shown in Step 4 and 5; here, the process of one representation is depicted for clarity. Then, they are used to make predictive distribution as shown in step 6.

%--------------------------------------------------------------------------
%page 3 outline fig
%--------------------------------------------------------------------------
\begin{figure*}[t!]
\centering
% {\includegraphics[width=0.99\linewidth]{Figures/03-methodology-explain01/bconvcnp_outline_v5.PNG}}   
%{\includegraphics[width=0.95\linewidth]{Figures/03-methodology-explain01/tmp2.PNG}}   
{\includegraphics[width=0.98\linewidth]{Figures/03-methodology-explain01/outline_v3.pdf}} 
\caption{\textr{Prediction procedure:} \textbf{Step 1:} Given context set $D^{c}$. \textbf{Step 2:} Consider the random stationary functions $\{\phi_{q}\}_{q=1}^{Q}$ of \cref{eqn:mixed_fourier}. \textbf{Step 3:} Assign the task-dependent kernel by \cref{eqn:latent_sample,eqn:mixedkernel} for the context set $D^{c}$ in Step 1, and then construct $N$ random representations $\{RE_{(n)}(D^{c}) (\bigcdot)\}_{n=1}^{N}$ in \cref{eqn:bayes_convdeepset}. \textbf{Step 4:} Discretize the representation as explained in \cref{eqn:finite_convdeepset}. \textbf{Step 5:} Map the discredited representation via CNN, i.e., ${\Phi^{\mathcal{B}}_{(n)}}(D^{c})(\bigcdot)$. \textbf{Step 6:} Smooth the mapped representations by \cref{eqn:smoothed}, and make prediction distribution by \cref{eqn:prediction}. For the Step 4 and 5, one random representation is depicted for clarity.}
\label{fig:main-illustration2}
\end{figure*}


Then, we consider the categorical latent variable $Z_{\text{cat}} = (z_1,..,z_Q)$ parameterized by the neural network as follows:
\begin{align}
q(Z_{\text{cat}} \ | \ D^c) = \mathrm{Cat} \left( Z_{\text{cat}} \ ; \ \mathrm{p}_{\mathrm{nn}}(D^{c}) \right) \label{eqn:latentcat},
\end{align}
where $\mathrm{p}_{\mathrm{nn}}: D^c \longrightarrow {\Delta}^{Q-1} $, with $Q$-dimension simplex ${\Delta}^{Q-1}$, denotes the parameter of categorical variable parameterized by the translate invariant neural network satisfying 
\begin{align}
\vspace{-2mm}
\mathrm{p}_{\mathrm{nn}} (T_{\tau}(D^{c})) = \mathrm{p}_{\mathrm{nn}}(D^{c})  \label{eqn:transinv_net},
\end{align}
where $T_{\tau}(D^{c}) {=} \left((x^{c}_{1}+\tau,y^{c}_1), .., (x^{c}_{N^{c}}+\tau,y^{c}_{N^{c}}) \right) $ denotes the $\tau$-translated context set defined in \cref{def:TE}. This $\mathrm{p}_{\mathrm{nn}} $ is designed to make the derived functional representation satisfy the TE, \textr{which will be stated in \cref{pro:Bayes_convdeepset}.} \textr{The structure of $\mathrm{p}_{\mathrm{nn}}$ in this work is described in Appendix A.2}. 

Using the kernels $\{k_q(\tau) \}_{q=1}^{Q}$ in \cref{eqn:basiskernel} and the latent variable $Z_{\mathrm{cat}}(D^{c})$ in \cref{eqn:latentcat}, we build the amortized latent stationary kernel depending on the context set $D^{c}$ as
\begin{align}
k(\tau) \ | \ Z_{\text{cat}}(D^{c}) = z_1 k_1(\tau)  \hspace{2mm} +  \hspace{2mm} \cdots  \hspace{2mm}  + \hspace{2mm} z_Q k_Q(\tau).
\label{eqn:mixedkernel}
\end{align}
\paragraph{Multi-channel Extension.}  The latent stationary kernel in \cref{eqn:mixedkernel} can be extended for multi-channel processes ($K$ channels) by considering $K$-th channel categorical variables $\{Z_{\text{cat}}^{k}(D^{c})\}_{k=1}^{K}$ with $Z_{\text{cat}}^{k}(D^{c}) {\sim} \mathrm{Cat}( \mathrm{p}^k (D^{c}) )$, where $\mathrm{p}^k (D^{c})$ denotes the amortized parameter for $k$-th channel.
\vspace{-2mm}
%\paragraph{Task-Dependent Stationary Prior}
\subsection{Bayesian Convolutional Deep sets.} 
\label{subsec:method3}
\vspace{-1mm}


Based on the latent stationary kernel in \cref{eqn:mixedkernel}, we build the random data representation, and the construct the Bayesian ConvDeepsets. \textr{To this end, we employ the path-wise sampling for GP posterior that constructs the sample function of GP posterior efficiently; this can reduce the computation cost of conventional posterior sampling by computing the prior function and update function of the data separately \citeb{wilson2020efficiently}.} Let $f(D^c)(\bigcdot)$ be the random data representation for the context set $D^c = \{(x^{c}_n,y^{c}_{n})\}_{n=1}^{N^c}$, and it can be represented
\vspace{-2mm}
\begin{align}
\hspace{-2mm}
\underbrace{ f(D^c)(\bigcdot) }_{ \substack{\mathrm{random \ data} \\ \mathrm{representation}} } & \coloneqq \hspace{3mm} 
\underbrace{\sum_{q=1}^{Q}\sqrt {z_q} \ \phi_q(\bigcdot) }_{\mathrm{prior \  term}} 
\hspace{.5mm} + \hspace{.5mm} 
\underbrace{\sum_{n=1}^{N^{c}} v_{n}  \ k(\bigcdot - x^{c}_{n} )}_{\mathrm{update \ term }}.
\label{eqn:randomfunctionalfeature}
\end{align}
% to assign the task-dependent stationary prior, i.e,
\textr{
For computing the prior, we construct the random samples $(z_{1},..,z_{Q})$ of the latent categorical variable of \cref{eqn:latentcat}, i.e.,  
\begin{align}
(z_{1},..,z_{Q})  \sim \mathrm{Cat} \left( Z_{\text{cat}} \ ; \ \mathrm{p}_{\mathrm{nn}}(D^{c}) \right)
\label{eqn:latent_sample}
\end{align}
by applying the Gumbel-softmax trick \citeb{jang2016categorical} to the output of $\mathrm{p}_{\mathrm{nn}}(D^{c})$. We construct $q$-the random stationary function $ \phi_q(\bigcdot)$, i.e., a sample function of GP prior using $q$-th kernel $k_q$, based on random Fourier feature (RFF) \citeb{rahimi2007random,jung2022efficient}, as 
\vspace{-2mm}
\begin{align}
 & \{w_{q,i}\}_{i=1}^{l} {\sim} N(0,I), \ \{s_{q,i}\}_{i=1}^{l} {\sim} p_{q}(s), \  \{b_{q,i}\}_{i=1}^{l} {\sim} U[0,2\pi],   \nonumber \\
 & \hspace{5mm} \phi_q(\bigcdot) = \sqrt{\frac{2}{l}} \sum_{i=1}^{l} w_{q,i} \cos{ ( 2 \pi \langle  s_{q,i}, \bigcdot \rangle + b_{q,i})} \label{eqn:mixed_fourier},   
\end{align}%\vspace{-1mm}
where $w_{q,i}$ denotes random weight samples, $s_{q,i}$ and $b_{q,i}$ denote the spectral points sampled from $p_{q}(s)$ and phase sampled from uniform distribution $U[0,2\pi]$, respectively.
}





% where \textb{\{$w_{q,i}\}_{i=1}^{l}$} denotes $l$ random weight samples. The $q(Z_{\text{Cat}} \ |\  D^{c})$ denotes the distribution of the amortized latent variable in \cref{eqn:latentcat}. The $\{p_{q}(s)\}_{q=1}^{Q}$ and $U[0,2\pi]$ denote the spectral density of the $k_q(\tau)$ in \cref{eqn:basiskernel} and the uniform distribution defined on $[0,2\pi]$, respectively. The $\{\phi_q(\bigcdot)\}_{q=1}^{Q}$ denotes the random stationary prior function of $\{k_q\}_{q=1}^{Q}$ kernels by using random Fourier feature (RFF) \citeb{rahimi2007random,jung2022efficient}. 


% In this procedure, we use the Gumbel-softmax trick \citeb{jang2016categorical}, for $Z_{\text{Cat}}$ in \cref{eqn:latentcat} and reparametrization trick \citeb{jung2022efficient} for the prior term in \cref{eqn:randomfunctionalfeature}. These tricks enables end-to-end training, based on the automatic differentiation.
% \vspace{-1mm}
% \begin{align}
%  & (z_{1},..,z_{Q})  \sim q(Z_{\text{Cat}} \ | \ D^{c}), \hspace{3mm}
%   \{w_{q,i}\}_{i=1}^{l} \sim N(0,I), \nonumber \\
%  &\{s_{q,i}\}_{i=1}^{l} \sim p_{q}(s), \hspace{3mm}
%  \{b_{q,i}\}_{i=1}^{l} \sim U[0,2\pi] , \hspace{1mm} q=1,..,Q   \nonumber  \\
%  &\phi_q(\bigcdot) = \sqrt{\frac{2}{l}} \sum_{i=1}^{l} w_{q,i} \cos{ ( 2 \pi \langle  s_{q,i}, \bigcdot \rangle + b_{q,i})} \label{eqn:mixed_fourier}.   
% \end{align}%\vspace{-1mm}
% The \textb{\{$w_{i}\}_{i=1}^{l}$} denotes $l$ random weight samples. The $q(Z_{\text{Cat}} \ |\  D^{c})$ denotes the distribution of the amortized latent variable in \cref{eqn:latentcat}. The $\{p_{q}(s)\}_{q=1}^{Q}$ and $U[0,2\pi]$ denote the spectral density of the $k_q(\tau)$ in \cref{eqn:basiskernel} and the uniform distribution defined on $[0,2\pi]$, respectively. The $\{\phi_q(\bigcdot)\}_{q=1}^{Q}$ denotes the random stationary prior function of $\{k_q\}_{q=1}^{Q}$ kernels by using random Fourier feature (RFF) \citeb{rahimi2007random,jung2022efficient}. 

For comping the update term for \cref{eqn:randomfunctionalfeature}, we first the expected of \cref{eqn:mixedkernel} as 
\vspace{-.5mm}
\begin{align}
 k(\bigcdot - x^{c}_{i} ) &= \mathbb{E}_{ q(Z_{\text{cat}} \ | \ D^{c} ) }
 [  k(\bigcdot - x^{c}_{i} ) \ | \ Z_{\text{cat}}(D^{c})  ]  \label{eqn:updateterm} 
\end{align}
where the latent random variable $Z_{\text{cat}}(D^{c})$ is integrated over $q(Z_{\text{cat}}  |D^{C})$. We compute the weight of smoothing term $v_{i}$,
\begin{align}
 v_{i} &= \left[  K(X^{c},X^{c}) {+} \sigma^{2}_{\epsilon}I  ) {}^{-1}
          \left(Y^{c} - \Psi(X^{c}) \right)  \right]_{i},  \label{eqn:updateterm-2}  
\end{align}
where $ K(X^{c},X^{c}) \in R^{N_c \times N_c} $ the Gram matrix of the expected kernel in \cref{eqn:updateterm}, and $\Psi(X^{c})$ denotes the 




and \textr{the values of stationary function on $X^{c}$}, i.e., $i$-th element of $\Psi(X^{c})W \in R^{N_c}$ is evaluated by the prior term in \cref{eqn:randomfunctionalfeature} on $x^c_{i}$. 

The update term of \cref{eqn:randomfunctionalfeature} reflects the data $Y^{c}$ on function output value $f(D^c)(\bigcdot)$ by smoothing the data information $v_{i}$ with the expected kernel $ k(\bigcdot - x^{c}_{i} )$.

The \textb{$v_{i}$} denotes $i$-th element of the inversion term using the expected Gram matrix 



%smooths the data $Y^{c}$ on any the function output 
%and 


% \textr{Roughly speaking, the \cref{eqn:randomfunctionalfeature} can be understood as the generalization of the data representation of $E(D^{c})$ in sense that the random prior function using the expected kernel of \cref{eqn:mixedkernel} as the covariance is reflected on the representation.}
\cref{eqn:randomfunctionalfeature} can be also approximated, i.e., $f(D^c)(\bigcdot) \approx$
\begin{align}
\hspace{-.5mm}
\alpha
\underbrace{  \sum_{q=1}^{Q} \sqrt{z_q}   \phi_   q(\bigcdot)}_{\text{prior term}} +
\Tilde{k} * 
\Big(
\underbrace{
\sum_{n=1}^{N^{c}} y^{c}_n   \delta (\bigcdot -  x^{c}_n ) 
}_{\text{data term}}
- 
\alpha
\underbrace{
\sum_{q=1}^{Q} \sqrt{z_q}  \phi_q(\bigcdot) 
}_{\text{prior term}}
\Big) \nonumber
\end{align}
for scalability, where the $\alpha \in (0,1)$ denotes the hyperparameter for controlling how much the stationary prior is reflected on $f(D^c)(\bigcdot)$. The $ \Tilde{k}$ denotes the truncated expected kernel in \cref{eqn:updateterm} with the finite length, and is used as the filter for smoothing the difference of data and prior values. \textr{This approximation reflects the stationary prior and the data term on the data representation as $f(D^c)(\bigcdot)$ in \cref{eqn:randomfunctionalfeature}.} In experiment, we validate that this alleviates the task ambiguity on the large-size image datasets empirically.


%\cref{eqn:randomfunctionalfeature}

% Additionally, we emphasize that the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D) (\bigcdot)$ has the following characteristic :
% \vspace{-1mm}
% \begin{itemize}[leftmargin=1em]
%     \vspace{-1mm}
%     \item \textbf{Flexibility:} The amortized latent stationary kernel \cref{eqn:mixedkernel} can assign the reasonable stationary prior if the target task can be modeled by the candidate of the stationary kernel $\{k_1,..,k_Q\}$. This is because $\{k_1,..,k_Q\}$ can construct any stationary kernel based on \cref{eqn:basiskernel}.
    
%     \vspace{-1mm}
%     \item \textbf{Generalization :} The random representation $f(D^{c})(\bigcdot)$ in \cref{eqn:randomfunctionalfeature} can be understood as the generalization of the data channel of $E(D^{c})$ in \cref{eqn:convdeepset}; note that if the random prior term is not considered and the RBF kernel is used for $f(D^{c})(\bigcdot)$, the $f(D^{c})(\bigcdot)$ represents the data channel of $E(D^{c})$. Thus, the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D) (\bigcdot)$ generalizes the ConvDeepsets the $\Phi (D) (\bigcdot)$.

    
%     \vspace{-0.5mm}
% \end{itemize}




Then, we can construct the random functional representation $RE(D) (\bigcdot)$ through the $f(D^{c})(\bigcdot)$ in \cref{eqn:randomfunctionalfeature}, and the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D^{c}) (\bigcdot) $ as the ConvDeepsets $\Phi (D^{c}) (\bigcdot) $ is constructed in \cref{pro:convdeepset} as follows:  
\vspace{-1mm}
\begin{align}
    \hspace{-0.5mm} 
       \underbrace{RE(D^{c}) (\bigcdot) }_{ \substack{ \mathrm{random \ functional} \\ \mathrm{representation} }    }  & =
    \Big[ \  
      \underbrace{\sum_{n=1}^{N^{c}}  k(\bigcdot -  x^{c}_n)}_{\mathrm{density}} 
          \hspace{3mm}  , \ 
         \underbrace{f(D^c)(\bigcdot) }_{ \substack{ \mathrm{random \ data} \\ \mathrm{representation}} }
          \
    \Big], \nonumber \\ 
 \underbrace{  \Phi^{\mathcal{B}} (D^{c}) (\bigcdot) }_{ \substack{ \mathrm{Bayes \ ConvDeepsets} \\ \mathrm{representation} }    }   & =
    \underbrace{ \rho}_{ \substack{ \mathrm{mapping \ via} \\ \mathrm{ CNN} } } 
    \circ 
    \underbrace{RE(D^{c}) (\bigcdot) }_{ \substack{ \mathrm{random  \ functional} \\ \mathrm{representation} }    }       
    \label{eqn:bayes_convdeepset} 
\end{align}


%  if the 
% e consider the translate invariant neural network satisfying 
% \begin{align}
% \mathrm{p}_{\mathrm{nn}} (T_{\tau}(D^{c})) = \mathrm{p}_{\mathrm{nn}}(D^{c}),
% \end{align}
We prove that the Bayesian ConvDeepsets still holds the translation equivariance (TE) in the following proposition.
\begin{proposition} 
\label{pro:Bayes_convdeepset}
Given the dataset $D=\{(x_n,y_n)\}_{n=1}^{N}$, if the Bayesian ConvDeepsets $\Phi^{\mathcal{B}} (D) (\bigcdot)$ is defined on the finite grid points, $\Phi^{\mathcal{B}} (D) (\bigcdot)$ is still translation equivariant \textr{in distribution sense}, i.e.,
\begin{align}
\Phi^{\mathcal{B}}  \circ (T_{\tau}(D)) \stackrel{d}{=}  T^{*}_{\tau} \circ (\Phi^{\mathcal{B}}(D)).
\label{eqn:te_probsense}
\vspace{-3mm}
\end{align}

\begin{proof}
The proof can be checked in \textr{Appendix A.3}.
\end{proof}
\vspace{-2mm}
\end{proposition}
% \textr{Roughly speaking,} the components of $f(D)(\bigcdot)$, defined by \cref{eqn:randomfunctionalfeature}, are consistently constructed in regardless of the translated dataset $T_{\tau}(D) = \{(x_n + \tau,y_n) \}_{n=1}^{N}$. The detailed proof can be checked in \textr{Appendix}.


\vspace{-2mm}





















\subsection{Prediction and Training}
\label{subsec:method4}


%\paragraph{Model.}
\paragraph{Prediction.} For the context set $D^{c}$ and target set $D^{t}$, 
the Bayesian ConvDeepsets can be used for computing predictive distribution $p(Y^{t}| X^{t}, D^{c} )$ as 
\begin{align}
& p(Y^{t}| X^{t}, D^{c} )  \label{eqn:prediction}\\
& =\int 
p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}  ) 
p(\Phi^{\mathcal{B}} | Z_{\text{Cat}},D^{c} )
\ p(Z_{\text{Cat}}| D^{c}  ) 
\ 
d \Phi^{\mathcal{B}}
d Z_{\text{Cat}}  \nonumber  \\
&\approx \frac{1}{N} \sum_{n=1}^{N} p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}_{(n)}  )  \nonumber
% {=} \frac{1}{N} \sum_{n=1}^{N} N(Y^{t}| \mu^{(n)}_{\text{nn}}(X^{t}), \sigma^{2(n)}_{\text{nn}}(X^{t})  ) \nonumber
\end{align}
where the $Z_{\text{Cat}}$ denotes the categorical latent variable of \cref{eqn:latentcat} for choosing the stationary kernel; the $\Phi^{\mathcal{B}}$ denotes the representation of the Bayes ConvDeepsets $\Phi^{\mathcal{B}}(D^{c})(\bigcdot)$ evaluated on finite grid  $ \{t_m\}_{m=1}^{M}$ (see \cref{eqn:finite_convdeepset}), and $\Phi^{\mathcal{B}}_{(n)}$ denotes $n$-th random function sampled from $p( \Phi^{\mathcal{B}})$. The $p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}_{(n)}  )$ is modeled as 
\begin{align}
p(Y^{t}| X^{t}, \Phi^{\mathcal{B}}_{(n)}  )= N(Y^{t}| \mu_{(n)}(X^{t}), \sigma^{2}_{(n)}(X^{t}) ),
\label{eqn:prediction}
\end{align}
where the $n$-th predictive mean $\mu_{(n)}(X^{t})$ and standard deviation $\sigma^{2}_{(n)}(X^{t})$ on the target inputs $X^{t}$ are obtained by mapping the smoothed features of $X^{t}$ and $n$-th sample function $\Phi^{\mathcal{B}}_{(n)}$, as explained in \cref{eqn:smoothed}, via the neural network.







% \begin{figure*}[t]
% %\begin{figure}[htp!]
% \centering
% \subfloat[RBF]
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_rbf_v1.pdf}}   \hspace{0.1mm} 
% \subfloat[ Matern-${\frac{5}{2}}$] 
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_matern_v1.pdf}}   
% \subfloat[Weakly periodic]
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_weaklyperiodic_v1.pdf}}  \hspace{0.1mm} 
% \subfloat[Sawtooth]
% {\includegraphics[width=0.24\linewidth]{Figures/05-experiments-task01-v2/datav1_sawtooth_v1.pdf}}   
% \caption{AAA}
% \label{fig:exp5-1:smallset_comparison}
% \end{figure*}






% \begin{figure*}[t]
% \subfloat[\label{fig:1d-singletask-a}  Spectral density]
% {\includegraphics[width=0.19\linewidth  ,height=2.40cm ]{Figures/05-experiments-task01/tmp0-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-b} RBF]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp1-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-c} Matern-${\frac{5}{2}}$]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp2-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-d} Weakly Periodic]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp3-datav1.pdf}} \hspace{0.1mm}
% \subfloat[\label{fig:1d-singletask-e} Sawtooth]
% {\includegraphics[width=0.19\linewidth ,height=2.40cm ]{Figures/05-experiments-task01/tmp4-datav1.pdf}}  
% \vspace{1mm}
% \subfloat[\label{fig:1d-singletask-f} Prediction with \textr{$N^c=15$} context points]
% % {\includegraphics[width=0.99\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx8_bidx4_nc15_k4.pdf}}
% {\includegraphics[width=0.99\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx32_bidx0_nc15_k5.pdf}}
% \caption{Stochastic processes modeling beyond training range (gray region $[4,8]$): \cref{fig:1d-singletask-a,fig:1d-singletask-b,fig:1d-singletask-c,fig:1d-singletask-d,fig:1d-singletask-e} denote the trained spectral density of \cref{eqn:basiskernel} and $p_{\mathrm{nn}}(D^{c})$ of \cref{eqn:transinv_net} for each process, and \cref{fig:1d-singletask-f} denotes the prediction for the task of each process.}
% \label{fig:1d-singletask-prediction}
% \end{figure*}
% \vspace{-1mm}



\begin{figure*}[t]
\subfloat[\label{fig:1d-singletask-a}  Spectral density]
{\includegraphics[width=0.19\linewidth  ,height=2.5cm ]{Figures/05-experiments-task01/density_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-b} RBF]
{\includegraphics[width=0.19\linewidth ,height=2.5cm ]{Figures/05-experiments-task01/rbf_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-c} Matern-${\frac{5}{2}}$]
{\includegraphics[width=0.19\linewidth ,height=2.5cm ]{Figures/05-experiments-task01/matern_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-d} Weakly Periodic]
{\includegraphics[width=0.19\linewidth ,height=2.5cm ]{Figures/05-experiments-task01/weaklyperiodic_datav1.pdf}} \hspace{0.1mm}
\subfloat[\label{fig:1d-singletask-e} Sawtooth]
{\includegraphics[width=0.19\linewidth ,height=2.5cm ]{Figures/05-experiments-task01/sawtooth_datav1.pdf}}  
\vspace{1mm}
\subfloat[\label{fig:1d-singletask-f} Predictive distribution of each baseline on each process \textr{($N^c=15$)} ]
% {\includegraphics[width=0.99\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx8_bidx4_nc15_k4.pdf}}
{\includegraphics[width=0.975\linewidth  ]{Figures/05-experiments-task01-v2/pred_1d_validx32_bidx0_nc15_k5.pdf}}
\caption{\textr{Stochastic processes modeling beyond training range (gray region $[4,8]$): \cref{fig:1d-singletask-a} denote the trained spectral density of \cref{eqn:basiskernel} with $Q=4$ kernels. \cref{fig:1d-singletask-b,fig:1d-singletask-c,fig:1d-singletask-d,fig:1d-singletask-e} denote the parameter of categorical variable, i.e., the output of $\mathrm{p}_{\mathrm{nn}}(D^{c})$ for 128 context set $\{D^{c}_{n}\}_{n=1}^{128}$ of each process. \cref{fig:1d-singletask-f} shows predictive distributions of the baselines on each process. 
}
}
\label{fig:1d-singletask-prediction}
\end{figure*}
\vspace{-2mm}
%64 context set $\{D^{c}_{n}\}_{n=1}^{128}$ of each process

% \caption{Stochastic processes modeling beyond training range (gray region $[4,8]$): \cref{fig:1d-singletask-a,fig:1d-singletask-b,fig:1d-singletask-c,fig:1d-singletask-d,fig:1d-singletask-e} denote the trained spectral density of \cref{eqn:basiskernel} and $p_{\mathrm{nn}}(D^{c})$ of \cref{eqn:transinv_net} for each process, and \cref{fig:1d-singletask-f} denotes the prediction for the task of each process.}

















% Let $\Theta$ be the learnable parameters for kernels $\{k_q\}_{q=1}^{Q}$ of \cref{eqn:basiskernel}, the noise parameters $\sigma_{\epsilon}$, $p_{\mathrm{nn}}$ of \cref{eqn:transinv_net}, and the CNN $\rho$ of \cref{eqn:bayes_convdeepset}. 

%variational inference \citeb{burda2016importance}

\paragraph{Training.} \textr{Let $\Theta = \{\theta_{\mathrm{kernels}}, \theta_{\mathrm{p_{\mathrm{nn}}}}, \theta_{\rho},\theta_{\mathrm{pred}}\}$ be the learnable parameters for kernels, the translate invariant network, the CNN, and the network for prediction}. Then, using meta-learning, we maximize the following objective w.r.t $\Theta$ :
\begin{align}
 \mathbb{E}_{D^{c},D^{t} \sim p(\mathcal{T})} 
 \bigl[
 \mathcal{L}_{\text{ll}}(\Theta ; D^{c}, D^{t})  - \beta \hspace{.2mm} \mathcal{L}_{\text{reg}}( \Theta ;D^{c}, D^{t}) 
 \bigr]
\label{eqn:tr_objective}
\end{align}
where $\mathcal{L}_{\text{ll}}(\Theta ; D^{c}, D^{t})$ denotes the log likelihood. The $\mathcal{L}_{\text{reg}}(\Theta;D^{c}, D^{t})$ denotes the regularizer that induces the network $\mathrm{p}_{\mathrm{nn}}(D^c)$ in \cref{eqn:latentcat} to assign the reasonable stationary prior depending on context set $D^c$.

The log likelihood $\mathcal{L}_{\text{ll}}(\Theta ; D^{c}, D^{t})$ is expressed as 
\begin{align}
\log{
\left(
 \frac{1}{N} 
 \sum_{n=1}^{N} \exp{ \left(  \sum_{i=1}^{N^{t}} \log{p \left(  y^{t}_{i}| x^{t}_{i}, \Phi^{\mathcal{B}}_{(n)}  \right)}  \right) }   
 \right)  
 },   \nonumber
\end{align}
which can be optimized in end-to-end manner based on the automatic differentiation by \citeb{jang2016categorical,jung2020approximate}.


The regularizer $\mathcal{L}_{\text{reg}}(\Theta;D^{c}, D^{t})$ is expressed as 
% \begin{align}
% \mathcal{L}_{\text{reg}}(\Theta;D^{c}, D^{t})= \mathrm{KL} \left( q(Z_{\text{cat}} \ | \  D^{c} )  \ || \  p (Z_{\text{cat}} \ | \  D^{c}, D^{t}  )  \right) \nonumber
% %\label{eqn:reg-kl-zat}
% \end{align}
\begin{align}
\mathrm{KL} \left( q(Z_{\text{cat}} \ | \  D^{c} )  \ || \  p (Z_{\text{cat}} \ | \  D^{c}, D^{t}  )  \right) \nonumber
%\label{eqn:reg-kl-zat}
\end{align}
where $q(Z_{\text{cat}} \ | \  D^{c} )$  denotes the amortized categorical variable defined in \cref{eqn:latentcat}. The $ p (Z_{\text{cat}} \ | \  D^{c}, D^{t} ) $ denotes the posterior distribution of $Z_{\text{cat}}$, which will be used as the prior distribution for training $q(Z_{\text{cat}} \ | \  D^{c} )$. Note that $p (Z_{\text{cat}} \ | \  D^{c}, D^{t} )$ can be computed only during training phase.

%e k-dimensional sample vectors y ∈ ∆k−1

The posterior $ p (Z_{\text{cat}} \ | \  D^{c}, D^{t}  )= \mathrm{Cat}(Z_{\text{cat}};\mathrm{p}_{\mathrm{prior}}  ) $ is computed with the parameter $\mathrm{p}_{\mathrm{prior}} \in {\Delta}^{Q-1} $ of which $q$-th element $(\mathrm{p}_{\mathrm{prior}})_{q} $ is defined as follows: 
\begin{align}
(\mathrm{p}_{\mathrm{prior}})_{q} = 
\frac{\mathrm{exp} \left( \log{p(Y^{t} | X^{t}, D^{c}, k_q)} \ / \  \tau_{0} \right)}
{\sum_{q=1}^{Q} \mathrm{exp} \left( \log{p(Y^{t} | X^{t}, D^{c}, k_q)} \ /\  \tau_{0} \right)}
\end{align}
where $\tau_{0}$ denotes the tempering parameters. The $q$-th marginal likelihood $p(Y^{t} | X^{t},D^{c}, k_q)$, using the $q$-th stationary kernel $k_q$, is computed as
\begin{align}
\hspace{-2.2mm}
p(Y^{t} | X^{t},D^{c}, k_q) = N( Y^{t} ;\hat{\mu}_{q}(X^{t}),\mathrm{Diag}(\hat{\Sigma}_{q}(X^{t})) ) 
\label{eqn:emp-gpposterior}
\end{align}
where $\hat{\mu}_{q}(X^{t}) \in R^{N_t}$ and $\mathrm{Diag}(\hat{\Sigma}_{q}(X^{t})) \in R^{N_t}$ denote the empirical predictive mean and diagonal covariance of the GP posterior distribution on target set $X^{t}$. The sample functions of GP posterior, described in \cref{eqn:randomfunctionalfeature}, are used. The derivation of training loss is explained in \textr{Appendix A.3}.






==> 04-relatedwork-v03.tex <==




\section{ \textr{Related Work}}




%\color{red}
% \paragraph{NP Family Models.} Neural process (NP) \citeb{garnelo2018neural} and Conditional neural process (CNP) \citeb{garnelo2018conditional} are the pioneering deep learning framework for modeling the stochastic process, i.e., the functions over the distribution. Later, many variants \citeb{vaswani2017attention,singh2019sequential,yoon2020robustifying,louizos2019functional} have been proposed to improve the NP and CNP.  
%\citeb{kawano2020group,holderrieth2021equivariant} 


\vspace{-2mm}
\paragraph{Comparison with ConvLNP.} Convolutional neural process (ConvLNP) \citeb{foong2020meta} considers the latent random variable into the ConvCNP to relax the conditional independence assumption of ConvCNP. To this end, ConvLNP employs the modified ConvDeepsets of which output is the sample of Gaussian distribution (latent), and those samples are used for prediction. However, training the ConvLNP is known to be difficult as compared to ConvCNP in Section 7, \citeb{gordon2021advances}. We hypothesize that this difficulty arises because (1) the latent variables are constructed from the ambiguous representation of ConvDeepsets, and (2) the inherent randomness of the latent variable prevents the model from fitting the task set well. On the other hand, the proposed method first constructs the multiple random representations of \cref{eqn:randomfunctionalfeature} via the task-dependent prior, and then those are mapped via CNN. This can compensate for ambiguous representation for the tasks, and thus leads the model to be trained well.
\vspace{-3mm}
\paragraph{Comparison with GPConvCNP.}
Gaussian Process Convolutional neural process (GPConvCNP) \citeb{petersen2021gp} uses the sample function of GP Posterior as the functional representation for generalization, which is similar approach with our work. However, the proposed method is distinct with following perspective; (1) our work is based on the path-wise sampling of GP posterior \citeb{wilson2020efficiently}, and explains how the ConvDeepsets can be generalized by adding stationary prior term. Also, we prove that the Bayesian ConvDeepsets still holds the TE as shown in \cref{pro:Bayes_convdeepset} and present the scalable approximation as well, (2) our work considers the task-dependent prior on the functional representation as described in, whereas the GPConvCNP consider the RBF kernel, and do not delve into how the chosen kernel function of GP affects the functional representation.

%\cref{eqn:transinv-net,eqn:cat-gpprob}




% considers the task-dependent prior on the functional representation as described in \cref{eqn:transinv-net,eqn:cat-gpprob}, whereas the GPConvCNP focused on improving the generalization of the ConvCNP, and do not delve into how the chosen kernel function of GP affects the functional representation and thus the performance of the GPConvCNP.




% whereas the GPConvCNP focused on improving the generalization of the ConvCNP, and do not delve into how the chosen kernel function of GP affects the functional feature and the performance of the GPConvCNP.




==> 04-relatedwork-v04.tex <==




% \section{ \textr{Related Work}}
% %\color{red}
% % \paragraph{NP Family Models.} Neural process (NP) \citeb{garnelo2018neural} and Conditional neural process (CNP) \citeb{garnelo2018conditional} are the pioneering deep learning framework for modeling the stochastic process, i.e., the functions over the distribution. Later, many variants \citeb{vaswani2017attention,singh2019sequential,yoon2020robustifying,louizos2019functional} have been proposed to improve the NP and CNP.  
% %\citeb{kawano2020group,holderrieth2021equivariant} 


% \vspace{-2mm}
% \paragraph{Comparison with ConvLNP.} Convolutional neural process (ConvLNP) \citeb{foong2020meta} considers the latent random variable into the ConvCNP to relax the conditional independence assumption of ConvCNP. To this end, ConvLNP employs the modified ConvDeepsets of which output is the sample of Gaussian distribution (latent), and those samples are used for prediction. However, training the ConvLNP is known to be difficult as compared to ConvCNP in Section 7, \citeb{gordon2021advances}. We hypothesize that this difficulty arises because (1) the latent variables are constructed from the ambiguous representation of ConvDeepsets, and (2) the inherent randomness of the latent variable prevents the model from fitting the task set well. On the other hand, the proposed method first constructs the multiple random representations of \cref{eqn:randomfunctionalfeature} via the task-dependent prior, and then those are mapped via CNN. This can compensate for ambiguous representation for the tasks, and thus leads the model to be trained well.
% \vspace{-3mm}
% \paragraph{Comparison with GPConvCNP.}
% Gaussian Process Convolutional neural process (GPConvCNP) \citeb{petersen2021gp} uses the sample function of GP Posterior as the functional representation for generalization, which is similar approach with our work. However, the proposed method is distinct with following perspective; (1) our work is based on the path-wise sampling of GP posterior \citeb{wilson2020efficiently}, and explains how the ConvDeepsets can be generalized by adding stationary prior term. Also, we prove that the Bayesian ConvDeepsets still holds the TE as shown in \cref{pro:Bayes_convdeepset} and present the scalable approximation as well, (2) our work considers the task-dependent prior on the functional representation as described in, whereas the GPConvCNP consider the RBF kernel, and do not delve into how the chosen kernel function of GP affects the functional representation.








%\color{red}
% \paragraph{NP Family Models.} Neural process (NP) \citeb{garnelo2018neural} and Conditional neural process (CNP) \citeb{garnelo2018conditional} are the pioneering deep learning framework for modeling the stochastic process, i.e., the functions over the distribution. Later, many variants \citeb{vaswani2017attention,singh2019sequential,yoon2020robustifying,louizos2019functional} have been proposed to improve the NP and CNP.  
%\citeb{kawano2020group,holderrieth2021equivariant} 

\vspace{-1mm}
\section{ \textr{Related Work}}
\vspace{-2mm}
We focus on some NP models designed for modeling stationary process, and compare them with the proposed method.
\vspace{-5mm}
\paragraph{Comparison with ConvLNP.} Convolutional latent neural process (ConvLNP) \citeb{foong2020meta} considers the latent variable into the ConvDeepsets for relaxing the conditional independence assumption of the ConvCNP. However, ConvLNP could have the same issue of the task ambiguity because it uses the structure of the ConvDeepsets. Also, its training is known to be more difficult in Section 7, \citeb{gordon2021advances}; we believe this difficulty arises because the latent variables are constructed from the ambiguous representation of ConvDeepsets, and the inherent randomness of the latent variable prevents the NP model from fitting the target set as well. On the other hand, the proposed method  constructs the multiple data representations of \cref{eqn:randomfunctionalfeature} via the task-dependent prior, and use them for modeling the task.







% To this end, ConvLNP employs the modified ConvDeepsets of which output is the sample of Gaussian distribution (latent), and those samples are used for prediction. However, training the ConvLNP is known to be difficult as compared to ConvCNP in Section 7, \citeb{gordon2021advances}. We hypothesize that this difficulty arises because (1) the latent variables are constructed from the ambiguous representation of ConvDeepsets, and (2) the inherent randomness of the latent variable prevents the model from fitting the task set well. On the other hand, the proposed method first constructs the multiple random representations of \cref{eqn:randomfunctionalfeature} via the task-dependent prior, and then those are mapped via CNN. This can compensate for ambiguous representation for the tasks, and thus leads the model to be trained well.


\vspace{-3mm}
\paragraph{Comparison with GPConvCNP.}
% Gaussian Process Convolutional neural process (GPConvCNP) \citeb{petersen2021gp} uses the sample function of GP Posterior as the functional representation for generalization, which is similar approach with our work. However, the proposed method is distinct with following perspective; (1) our work is based on the path-wise sampling of GP posterior \citeb{wilson2020efficiently}, and explains how the ConvDeepsets can be generalized by adding stationary prior term. Also, we prove that the Bayesian ConvDeepsets still holds the TE as shown in \cref{pro:Bayes_convdeepset} and present the scalable approximation as well, (2) our work considers the task-dependent prior on the functional representation as described in, whereas the GPConvCNP consider the RBF kernel, and do not delve into how the chosen kernel function of GP affects the functional representation.

GPConvCNP \citeb{petersen2021gp} uses the sample function of GP Posterior, with RBF kernel, as the functional representation, which is similar approach with our work. However, our work focuses more on generalizing the ConvDeepsets in Bayesian way; 1) we propose how to impose the task-dependent prior, 2) prove that the Bayesian ConvDeepsets still holds the TE as shown in \cref{pro:Bayes_convdeepset}, and 3) present the scalable approximation as well.


% However, the proposed method is distinct with following perspective; (1) our work is based on the path-wise sampling of GP posterior \citeb{wilson2020efficiently}, and explains how the ConvDeepsets can be generalized by adding stationary prior term. Also, we prove that the Bayesian ConvDeepsets still holds the TE as shown in \cref{pro:Bayes_convdeepset} and present the scalable approximation as well, (2) our work considers the task-dependent prior on the functional representation as described in, whereas the GPConvCNP consider the RBF kernel, and do not delve into how the chosen kernel function of GP affects the functional representation.




% considers the task-dependent prior on the functional representation as described in \cref{eqn:transinv-net,eqn:cat-gpprob}, whereas the GPConvCNP focused on improving the generalization of the ConvCNP, and do not delve into how the chosen kernel function of GP affects the functional representation and thus the performance of the GPConvCNP.




% whereas the GPConvCNP focused on improving the generalization of the ConvCNP, and do not delve into how the chosen kernel function of GP affects the functional feature and the performance of the GPConvCNP.




==> 05-experiments-table-01.tex <==



% \citeb{kim2018attentive}, \citeb{gordon2019convolutional}, \citeb{foong2020meta}, \citeb{petersen2021gp},\citeb{petersen2021gp}

\vspace{-2mm}
\begin{table*}[htp!]
    \caption{ \small Test log likelihood ($\uparrow$: better) of target sets that are sampled outside training range. }
    \label{tab:1d-singletask}
    \centering
    \resizebox{0.87\linewidth}{!}{ 
    \begin{tabular}{ l@{\hspace{2mm}} r@{\hspace{5mm}}  c@{\hspace{5mm}}c@{\hspace{5mm}} c@{\hspace{5mm}}c@{\hspace{5mm}} }
    \toprule
    %& & \multicolumn{5}{c}{\textbf{BatchEns << DeepEns (ResNet-32 on CIFAR-10)}} \\
    %\cmidrule(r){3-7}
    %Method                            &  \# Params & \gls{acc} ($\uparrow$) & \gls{nll} ($\downarrow$) & \gls{bs} ($\downarrow$) & %\gls{ece} ($\downarrow$) & \gls{dee} ($\uparrow$) \\
    
    Model          & $\#$Params     &      RBF &  Matern-${\frac{5}{2}}$ & Weakly Periodic  & Sawtooth \\
    \midrule
    %\multicolumn{6}{l}{\textsc{$M=28 \ (Q=7,m=4)$}} \\[1mm] 
    %\multicolumn{6}{l}{\textbf{Small number of context set} is used for training ($U([5,25])$) } \\[1mm] 
    %\multicolumn{6}{l}{\textbf{Training with the small number of context set - $\mathcal{U}([5,25])$ }} \\[.75mm] 
    %\multicolumn{6}{l}{Training with \textbf{the small number of context set} - $U([5,25])$ } \\[.5mm] 
    \multicolumn{6}{l}{\textbf{The small number of context set - $\mathcal{U}([5,25])$ }} \\[.75mm] 
    
    % CNP \citeb{garnelo2018conditional} &  
    % \textr{$50876$} & 
    %  &
    %  &
    %  &
    % \\

 %(-1.09, 0.02)  (-2.07, 0.02)  (-1.59, 0.02)  (-0.54, 0.01) 
 %166274,50652,50732,50649,50649,51069
   ANP &  
    $166274$ & 
    $\text{-} 1.09 \spm{0.02} $ &
    $\text{-} 2.07 \spm{0.02} $ &
    $\text{-} 1.59 \spm{0.02} $ &
    $\text{-} 0.54 \spm{0.01} $ \\
    
    ConvCNP   &  
    $50652$ & 
    $\textbf{0.40} \spm{0.01} $ &
    $\text{-}0.85 \spm{0.01} $ &
    $\text{-}1.28 \spm{0.02} $ &
    $0.50 \spm{0.01} $ \\
    
    ConvLNP   &  
    $50732$ & 
    $\text{-}0.61 \spm{0.02} $ &
    $\text{-}1.25 \spm{0.01} $ &
    $\text{-}1.28 \spm{0.01} $ &
    $\text{-}0.01 \spm{0.01} $ \\
    
    GPConvCNP-RBF   &  
    $50649$ & 
    $0.34 \spm{0.01} $ &
    $\text{-}\textbf{0.73} \spm{0.01} $ &
    $\text{-}1.13 \spm{0.01} $ &
    $0.34 \spm{0.01} $ \\
    
    GPConvCNP-SM   &  
    $50649$ & 
    $0.38 \spm{0.01} $ &
    $\text{-}0.76 \spm{0.01} $ &
    $\text{-}\textbf{1.04} \spm{0.01} $ &
    $0.36 \spm{0.01} $ \\
    
    
    \textb{Proposed}  &  
    $51069$ & 
    $\textbf{0.40} \spm{0.01} $ &
    $\text{-}0.77 \spm{0.01} $ &
    $\text{-}\textbf{1.04} \spm{0.01} $ &
    $\textbf{0.52} \spm{0.01} $ \\
    
    

% modelname: anp                            		 numparams:166274
% modelname: base                           		 numparams:50652
% modelname: baselatent                     		 numparams:50732
% modelname: cnp                            		 numparams:66818
% spikeslab version 7 with tempering 0.1
% modelname: gpdep                          		 numparams:51069
% modelname: gpind                          		 numparams:50649
% modelname: gpind                          		 numparams:50649
    
% ----------------------------------------------------------------------------------------------------
% datav: 1, small dataset
% ----------------------------------------------------------------------------------------------------
% inrange datav 1
%                               rbf         matern weaklyperiodic  \
% anpdeeprunv1         (-0.03, 0.01)  (-1.01, 0.01)  (-1.52, 0.02)   
% basedeeprunv1          (0.4, 0.01)  (-0.85, 0.01)  (-1.28, 0.02)   
% baselatentdeeprunv1  (-0.62, 0.02)  (-1.25, 0.01)  (-1.28, 0.01)   
% cnpdeeprunv1         (-0.03, 0.01)  (-1.41, 0.01)  (-1.22, 0.02)   
% gpdepdeeprunv1        (0.39, 0.01)  (-0.78, 0.01)  (-1.04, 0.01)   
% gpinddeeprunv1        (0.33, 0.01)  (-0.73, 0.01)  (-1.12, 0.01)   
% gpinddeeprunv3        (0.38, 0.01)  (-0.76, 0.01)  (-1.04, 0.01)   

%                           sawtooth  
% anpdeeprunv1          (0.25, 0.01)  
% basedeeprunv1          (0.5, 0.01)  
% baselatentdeeprunv1  (-0.01, 0.01)  
% cnpdeeprunv1          (-0.22, 0.0)  
% gpdepdeeprunv1        (0.51, 0.01)  
% gpinddeeprunv1        (0.33, 0.01)  
% gpinddeeprunv3        (0.35, 0.01)  


% outrange datav 1
%                               rbf         matern weaklyperiodic  \
% anpdeeprunv1         (-1.09, 0.02)  (-2.07, 0.02)  (-1.59, 0.02)   
% basedeeprunv1          (0.4, 0.01)  (-0.84, 0.02)  (-1.31, 0.02)   
% baselatentdeeprunv1  (-0.61, 0.02)  (-1.25, 0.01)  (-1.27, 0.01)   
% cnpdeeprunv1         (-1.31, 0.04)   (-1.6, 0.02)  (-1.55, 0.02)   
% gpdepdeeprunv1         (0.4, 0.01)  (-0.76, 0.01)  (-1.04, 0.01)   
% gpinddeeprunv1        (0.34, 0.01)  (-0.72, 0.01)  (-1.12, 0.01)   
% gpinddeeprunv3        (0.38, 0.01)  (-0.75, 0.01)  (-1.04, 0.01)   


%                           sawtooth  
% anpdeeprunv1         (-0.54, 0.01)  
% basedeeprunv1         (0.51, 0.01)  
% baselatentdeeprunv1   (-0.0, 0.01)  
% cnpdeeprunv1         (-0.81, 0.01)  
% gpdepdeeprunv1        (0.52, 0.01)  
% gpinddeeprunv1        (0.34, 0.01)  
% gpinddeeprunv3        (0.35, 0.01)  
















    
    \midrule
    %\multicolumn{6}{l}{\textsc{$M=28 \ (Q=7,m=4)$}} \\[1mm] 
    %\multicolumn{6}{l}{\textbf{Training with the large number of context set - $\mathcal{U}([10,50])$ }} \\[.75mm]
    %\multicolumn{6}{l}{Training with \textbf{the large number of context set} - $U([10,50])$ } \\[.5mm] 
    \multicolumn{6}{l}{\textbf{The large number of context set - $\mathcal{U}([10,50])$ }} \\[.75mm] 
    
    %\hline
%   CNP \citeb{garnelo2018conditional} &  
%     \textr{$50876$} & 
%      &
%      &
%      &
%     \\
 

   %(-2.86, 0.09)   (-4.16, 0.09)   (-2.31, 0.04)    (-0.76, 0.01) 
   ANP &  
    $166274$ & 
    $\text{-} 2.86 \spm{0.09} $ &
    $\text{-} 4.16 \spm{0.09} $ &
    $\text{-} 2.31 \spm{0.04} $ &
    $\text{-} 0.76 \spm{0.01} $ \\
    
    ConvCNP  &  
    $50652$ & 
    $0.54 \spm{0.01} $ &
    $\text{-} 0.31 \spm{0.01} $ &
    $\text{-}0.95 \spm{0.01} $ &
    $0.65 \spm{0.01} $ \\
    
    ConvLNP &  
    $50732$ & 
    $\text{-}0.61 \spm{0.02} $ &
    $\text{-}1.14 \spm{0.01} $ &
    $\text{-}1.28 \spm{0.01} $ &
    $\text{-}0.09 \spm{0.01} $ \\
    %baselatentdeeprunv1  (-0.61, 0.02)  (-1.14, 0.01)  (-1.29, 0.01)  (-0.1, 0.01)

    GPConvCNP-RBF  &  
    $50649$ & 
    $0.49 \spm{0.01} $ &
    $\text{-}0.30 \spm{0.01} $ &
    $\text{-}1.04 \spm{0.01} $ &
    $0.40 \spm{0.01} $ \\
    
    GPConvCNP-SM  &  
    $50649$ & 
    $\textbf{0.58} \spm{0.00} $ &
    $\text{-}\textbf{0.27} \spm{0.01} $ &
    $\text{-}\textbf{0.80} \spm{0.01} $ &
    $\textbf{0.73} \spm{0.01} $ \\


    \textb{Proposed}  &  
    $51069$ & 
    $0.55 \spm{0.01} $ &
    $\text{-}0.30 \spm{0.01} $ &
    $\text{-}0.90 \spm{0.01} $ &
    $0.61 \spm{0.01} $ \\
    
    
  \bottomrule    
\end{tabular}}

\end{table*}






% ----------------------------------------------------------------------------------------------------
% datav: 2, with large dataset
% ----------------------------------------------------------------------------------------------------
% inrange
%                               rbf         matern weaklyperiodic  \
% anpdeeprunv1          (0.38, 0.01)  (-0.64, 0.02)  (-1.47, 0.02)   
% basedeeprunv1         (0.54, 0.01)  (-0.31, 0.01)  (-0.95, 0.01)   
% baselatentdeeprunv1  (-0.66, 0.02)  (-1.15, 0.01)  (-1.28, 0.01)   
% cnpdeeprunv1           (0.2, 0.01)  (-1.33, 0.02)  (-1.13, 0.01)   
% gpdepdeeprunv1        (0.56, 0.01)   (-0.3, 0.01)  (-0.91, 0.01)   
% gpinddeeprunv1        (0.48, 0.01)   (-0.3, 0.01)  (-1.04, 0.01)   
% gpinddeeprunv3        (0.57, 0.01)  (-0.28, 0.01)  (-0.82, 0.01)   

%                           sawtooth  
% anpdeeprunv1          (0.54, 0.01)  
% basedeeprunv1         (0.65, 0.01)  
% baselatentdeeprunv1  (-0.09, 0.01)  
% cnpdeeprunv1          (-0.19, 0.0)  
% gpdepdeeprunv1        (0.61, 0.01)  
% gpinddeeprunv1        (0.39, 0.01)  
% gpinddeeprunv3        (0.73, 0.01)  


% outrange
%                                 rbf          matern  weaklyperiodic  \
% anpdeeprunv1          (-2.86, 0.09)   (-4.16, 0.09)   (-2.31, 0.04)   
% basedeeprunv1          (0.55, 0.01)    (-0.3, 0.01)   (-0.96, 0.01)   
% baselatentdeeprunv1    (-0.6, 0.02)   (-1.14, 0.01)   (-1.29, 0.01)   
% cnpdeeprunv1         (-27.32, 0.76)  (-26.01, 0.36)  (-33.89, 0.61)   
% gpdepdeeprunv1         (0.57, 0.01)   (-0.29, 0.01)    (-0.9, 0.01)   
% gpinddeeprunv1         (0.49, 0.01)   (-0.29, 0.01)   (-1.03, 0.01)   
% gpinddeeprunv3          (0.59, 0.0)   (-0.27, 0.01)    (-0.8, 0.01)   


%                           sawtooth  
% anpdeeprunv1         (-0.76, 0.01)  
% basedeeprunv1         (0.65, 0.01)  
% baselatentdeeprunv1   (-0.1, 0.01)  
% cnpdeeprunv1         (-6.49, 0.05)  
% gpdepdeeprunv1         (0.6, 0.01)  
% gpinddeeprunv1         (0.4, 0.01)  
% gpinddeeprunv3        (0.74, 0.01) 







==> 05-experiments-v05-part04.tex <==

\subsection{Predator-Pray model} % (Sim2Real)
\label{subsec:exp4}

We conduct the predator-pray benchmark experiment conducted in \citeb{gordon2019convolutional,petersen2021gp,lee2020bootstrapping}; the NP models are first trained on the synthetic dataset simulated by a Lotka-Volterra differential equation \citeb{lotka2002contribution}, and then predict the real-world dataset (Hudson’s Bay hare-lynx data). Further details of settings and additional results are reported in \textb{Appendix A.4}.

%{\includegraphics[width=0.48\linewidth,height=2.75cm]
\begin{figure}[H]
\subfloat[\label{fig:predpray-a} simulated set]
{\includegraphics[width=0.48\linewidth]{Figures/05-experiments-task03/simulation_comparison_varyingcontext_datav2.pdf}} \hspace{1mm}  
\subfloat[\label{fig:predpray-b} real set]
{\includegraphics[width=0.48\linewidth]{Figures/05-experiments-task03/real_comparison_varyingcontext_datav2.pdf}}  
\caption{{Prediction Results on simulated and real dataset;}}
\end{figure}



\cref{fig:predpray-a,fig:predpray-b} describes the mean and one-standard error of the test log likelihood for 1024 tasks of simulated and real datasets, respectively; we consider $N^{c}\in \{10,...,80\}$ context points. These figures imply that for small $N^{c}\in \{20,..,70\}$ context data points, task-dependent prior could help improve the prediction performance by using the different prior depending on $N^{c}$ context data points.







%\cref{appendix:pray-predator}.

% \vspace{-1mm}
% %\input{05-experiments-figure-06}
% \vspace{-1mm}


% \begin{figure*}[htp!]
% %\begin{figure*}[t]
% %\hspace{-5mm}
% \begin{minipage}[c]{.5\textwidth}
% \centering
% \subfloat[\label{fig:predpray-a} simulated set]
% {\includegraphics[width=0.48\linewidth,height=2.75cm]{Figures/05-experiments-task03/simulation_comparison_varyingcontext_datav2.pdf}} \hspace{.1mm}  
% \subfloat[\label{fig:predpray-b} real set]
% {\includegraphics[width=0.48\linewidth,height=2.75cm]{Figures/05-experiments-task03/real_comparison_varyingcontext_datav2.pdf}} \hspace{5mm}  
% \end{minipage}
% \begin{minipage}[c]{.5\textwidth}
% \centering
% \subfloat[\label{fig:predpray-c} spectral density]
% {\includegraphics[width=0.44\linewidth,height=2.75cm]{Figures/05-experiments-task03/real_comparison_varyingcontext_datav2_density.pdf}} \hspace{.1mm}  
% \subfloat[\label{fig:predpray-d} $p_{\mathrm{traninv-nn}}$ \cref{eqn:transinv-net}]
% {\includegraphics[width=0.52\linewidth,height=2.75cm]{Figures/05-experiments-task03/real_comparison_varyingcontext_datav2_prob.pdf}} 
% \end{minipage}
% %\caption{\textr{Sawtooth}}
% \caption{{Results on Predator-pray model; we use 4 basis stationary kernels, and only 2 kernels are actively assigned. Thus, the spectral densities of the corresponding kernels and the projected $p_{\mathrm{traninv}\textrm{-}\mathrm{nn}} \in R^{2}_{+}$ are reported in  \cref{fig:predpray-c,fig:predpray-d}, respectively.}}
% \end{figure*}



==> 06-discussion-v02.tex <==
%\section{Discussion}


% \paragraph{Summary.} We propose a Bayesian Convolutional Deep sets that uses task-dependent stationary prior to alleviate the potential problem of the Convolutional Deep sets that arises for given the small number of context data points. We have verified that the proposed methodology can overcome the targeted issue through the experiments with synthetic and real datasets.

\vspace{-1mm}
\section{Limitation}
\label{sec:discuss}

\vspace{-1mm}

We have experienced the following limitations: (1) If a targeted process could not be modeled by stationary process, the proposed method may not be helpful to model targeted process, because the Bayesian convolutional deep sets employ the stationary prior as a inductive bias, (2) Training the NP model using the Bayesian convolutional deep sets requires more training time because it employs the multiple random representations (trainable), which requires more computations in training, compared to the single representation of ConvCNP and ConvLNP; in experiments, we have experienced that training the proposed NP model takes about 2-times longer than that of ConvLNP on average.







% \paragraph{Limitation.} 
% %vspace{-1mm}
% \begin{itemize}[leftmargin=1em]
%     \vspace{-1mm}
%     \item If a targeted process could not be modeled by stationary process, the proposed method
%     may not be helpful to model targeted process, because the Bayesian convolutional deep sets employ the stationary prior as a inductive bias.
    
%     \vspace{-.25mm}
%     \item Training the NP model using the Bayesian convolutional deep sets takes more training time because it employs the multiple random representations (trainable) that requires more computations in training, compared to the single deterministic representation for ConvCNP and ConvLNP; in our experiments, we have experienced that training the proposed NP model takes about 2-times longer than that of ConvLNP on average.
% \end{itemize}















